A Plug-and-Play Physical Motion Restoration Approach for In-the-Wild High-Difficulty Motions

Extracting physically plausible 3D human motion from videos is a critical task. Although existing simulation-based motion imitation methods can enhance the physical quality of daily motions estimated from monocular video capture, extending this capability to high-difficulty motions remains an open challenge. This can be attributed to some flawed motion clips in video-based motion capture results and the inherent complexity in modeling high-difficulty motions. Therefore, sensing the advantage of segmentation in localizing human body, we introduce a mask-based motion correction module (MCM) that leverages motion context and video mask to repair flawed motions, producing imitation-friendly motions; and propose a physics-based motion transfer module (PTM), which employs a pretrain and adapt approach for motion imitation, improving physical plausibility with the ability to handle in-the-wild and challenging motions. Our approach is designed as a plug-and-play module to physically refine the video motion capture results, including high-difficulty in-the-wild motions. Finally, to validate our approach, we collected a challenging in-the-wild test set to establish a benchmark, and our method has demonstrated effectiveness on both the new benchmark and existing public datasets.https://physicalmotionrestoration.github.io

==> backup/Intro_1110.tex <==
\section{Introduction}
\label{sec:intro}


Our goal is to obtain physically plausible 3D human motions from monocular videos, including challenging actions such as gymnastics and head flips. 
This would supply the animation and film industries with high-quality 3D motion assets and meet the demand for large-scale 3D motion datasets in virtual human and robotics research.
With technological advancements, monocular video-based motion capture algorithms provide a fast and convenient pipeline for obtaining kinematically accurate motion. However, these methods lack dynamic modeling, leading to physical issues like self-penetration and foot sliding. Additionally, due to the long-tail distribution of challenging actions and motion blur, these methods struggle to accurately capture complex movements.

Physical plausible 3D human motion is in high demand across various fields, including virtual reality, game, animation industries, and academic research on virtual humans and robotics \cite{colombel2020physically,erickson2020assistive,mehta2017vnect}. With technological advancements, monocular video-based motion capture algorithms provide a fast and convenient pipeline for obtaining kinematically accurate motion \cite{wang2024tram,shen2024world,shin2024wham}, with the ability to capture high-difficulty motions like backflip and aerial tumbling. 
However, these methods inherently lack dynamic modeling, resulting in significant physical unrealisms such as floating, foot sliding, self-intersections, and ground penetration, things get worse when facing high-difficulty motions.

To enhance physical realism, learning-based methods introduce carefully designed kinematic constraints \cite{zanfir2018monocular,zhang2021learning,zhang2020perceiving,huang2022capturing} or construct a dynamic model to predict the physical parameters \cite{tripathi20233d,li2022d,gartner2022trajectory,xie2021physics}. However, these methods depend heavily on 3D annotations and the simplified dynamic equations struggle to handle high-difficulty motions. Physic-based motion imitation methods learn motion control policy to imitate the reference motion (video motion capture results) at a physically simulated environments to enhance physical plausibility. \cite{yuan2021simpoe,shimada2020physcap,gong2022posetriplet,gartner2022differentiable}. However, as shown in Fig \ref{fig:motivation} (b), when flaw motions occur in reference motion, short-term chaotic frames directly lead to the failure of the physical simulation. Also, as shown in Fig \ref{fig:motivation} (c),  even the state-of-the-art motion imitation method \cite{luo2023perpetual} fails when facing high-difficulty motions that rarely appear in existing motion priors. 
Thus, although many methods have performed well in capturing physical motions from video, achieving the physical restoration of high-difficulty motions is still an open challenge. 
Regarding this, we propose to design a plug-and-play motion restoration model to transform high-difficulty motions estimated by monocular video motion capture algorithms into physically realistic motions while preserving consistency with the original video.

The emergence of flaw motion (Fig \ref{fig:motivation} b) is mainly because high-difficulty motions often involve rapid movement and extreme poses, it is hard for motion capture algorithms to integrate generate and exhibit short periods of chaos. Since flaw motion only occurs over a short time and is surrounded by rich contextual information, interpolation and replacement of flaw motion can be used to correct the motion, avoiding the confrontation of flaw motion by the physical simulator. Therefore, we propose a mask-conditioned correction module (MCM) to repair the short-term flawed motions and ensure motion continuity. Guided by the rich shape and motion information provided by the original motion context and segmentation mask, we regenerate contextually consistent and reasonable motions to replace the flawed motion, allowing the entire motion sequence to be accurately and fully mapped into the physical space.

The failure to simulate high-difficulty motions (Fig \ref{fig:motivation} c) can be attributed to the generalization limitations of current physical simulation methods. Current human motion datasets still exhibit a long-tail distribution (with high-difficulty motion being rare), and the lack of motion priors makes it difficult for simulation methods to completely transfer complex motions into the physical space. Additionally, a single controller struggles to generalize across a diverse range of high-difficulty movements, facing significant catastrophic forgetting issues, where rapid loss of old knowledge occurs when learning new skills \cite{luo2023perpetual}. Therefore, we propose a reinforcement learning-based test-time adaptation strategy (RL-TTA) that enables targeted adjustments during testing for specific action segments. This strategy can effectively bridge the distribution gap between in-the-wild motions and training data.
% , thereby enhancing generalization capabilities. 
With the ability to track unseen motions, we design a set of adaptation settings for the RL-TTA strategy, making it possible to restore even in-the-wild and highly difficult motions. 


Through our proposed novel MCM and RL-TTA strategies, we successfully address the failure issues of flaw motion and complex motion simulation, achieving physical authenticity restoration in high-difficulty motions while faithfully retaining the original movements. It is worth mentioning that without additional training, our method can be conveniently integrated into any video motion capture method, directly repairing in-the-wild and high-difficulty motions.


% such as adding motion smoothing loss to address jitter and foot optimization loss to mitigate foot sliding and ground penetration. These methods require meticulous tuning of the weights for different loss functions and, fundamentally, do not account for the dynamic characteristics of motion, thus failing to fully resolve the physical realism problem.
% Other approaches construct a dynamic model of the human body and then train a network to predict the physical parameters required by the dynamic model \cite{tripathi20233d,li2022d,gartner2022trajectory,xie2021physics}. However, these methods often depend heavily on 3D annotated videos and struggle with generalization, particularly when dealing with complex, high-difficulty motions. Recently, PhysPT \cite{zhang2024physpt} has shown exceptional performance in optimizing standard movements but still lacks an understanding of the distribution and physical principles for complex motions, requiring substantial motion priors for effective operation. However, obtaining realistic data for high-difficulty movements remains a significant challenge.
% % heavily on 3D annotated videos and struggle with generalization. 
% % \lrh{How does the method based on dynamic model perform in solving the motion quality problems? And what other problems remain?}
% Due to the complexity of dynamic models, these approaches often oversimplify dynamic equations, leading to insufficient physical realism. Therefore, to better enhance the physical realism of motion, some methods utilize physically simulated environments and learn motion control strategies within such a virtual physical world to ensure physical realism \cite{yuan2021simpoe,shimada2020physcap,gong2022posetriplet,gartner2022differentiable}. They introduce a motion tracking task: given a reference motion clip, the goal of motion tracking is to reproduce the desired motion in a physically simulated environment.
% This approach allows for obtaining physically realistic 3D motions from monocular video in a two-stage process. The first stage uses kinematic methods to estimate pose-accurate motions, while the second stage employs motion tracking as a post-processing model to enhance the physical realism of the motion. This two-stage design effectively avoids the trade-off of modeling both kinematics and dynamics in a single model, demonstrating excellent ability to improve the physical quality of motion. 

% {\color{red}Our goal is to efficiently obtain high-quality, realistic motions while significantly reducing the high costs associated with traditional motion capture.}

% Inspired by motion tracking, we aim to design a plug-and-play motion restoration post-processing model to transform motion estimated by monocular video motion capture algorithms into physically realistic motions while preserving consistency with the original video. This task is challenging primarily in the following two aspects:
% \textbf{(1) Dynamics generalization limits:} Current video motion capture algorithms perform well in wild videos and can capture remarkably high-difficulty motions like backflips and Thomas flares. However, existing motion tracking algorithms require meticulous parameter tuning of the controllers \cite{zhang2024physpt}, which can lead to poor performance in wild motions. Additionally, a single controller struggles to generalize across a diverse range of high-difficulty movements, facing significant catastrophic forgetting issues, where rapid loss of old knowledge occurs when learning new skills \cite{luo2023perpetual}.
% \textbf{(2) Kinematics flaw motions:} We observed that motion captured from videos can produce short-term catastrophic errors when estimating challenging movements. Certain flawed motions significantly impact the motion-tracking process, as brief motion breakdowns can easily lead to failure in the simulation.  Moreover, since humans are highly sensitive to short-time discrepancies in motion, this flaw can severely impact motion quality in practical applications.
% % , frequently resulting in simulation failures,
% % Current motion tracking algorithms struggle to correct complex actions like backflips and Thomas flares. This difficulty arises, on the one hand, due to the complex dynamic characteristics of these motions, which make it challenging to train an effective control strategy for correction; on the other hand, monocular motion capture algorithms often produce catastrophic errors when estimating these challenging actions, further hindering the final output of reasonable motions.
% To tackle these challenges, 
% we propose a plug-and-play motion restore model that enhances the physical plausibility of motions while faithfully retaining the original movements. 
% A physical transfer module is introduced to enhance the physical realism of motion by simulation, along with an RL-based test time adaptation strategy to improve the in-the-wild motion generalization ability and encourage the tracking of high-difficulty motions. Additionally, a mask-conditioned correction module is proposed to handle occasional chaotic frames in the original motion, thereby enhancing the robustness of our restore model.
% % Based on motion tracking, we propose a physical transfer module to enhance the physical realism of motion and design additional training strategies and reward functions to improve the tracking of complex actions. Additionally, we introduce an RL-based test time adaptation strategy to improve generalization, along with a mask-based correction module to handle occasional chaotic frames in the given motion, thereby enhancing robustness.
% % Additionally, we are committed to providing a more cost-effective and efficient solution for motion capture by building on current video motion capture techniques. 
% % Our goal is to quickly obtain high-quality, realistic motions while significantly reducing the high costs associated with traditional motion capture.
% \textbf{For physical motion restoration}, the physical transfer module (PTM) is responsible for applying physical constraints to the original motions with a physics simulator.
% Specifically, using both large-scale video motion capture data and precise mocap data, we trained a powerful motion-tracking policy that controls the character agent in the simulator to track physically implausible motion captured from video. 
% This pre-trained module encompasses rich motion priors, enabling it to restore the physical plausibility of noisy motions effectively. 
% % However, it still faces challenges when dealing with in-the-wild movements and high-difficulty motions.
% \textbf{For Dynamics generalization limits}, 
% % {\color{red}the trial-and-error nature of reinforcement learning suggests we envision the potential for test-time adaptation without the need for additional manual annotations. Consequently}
% we propose a reinforcement learning-based test-time adaptation strategy (RL-TTA) that enables targeted adjustments during testing for specific action classes or segments. This strategy can effectively bridge the distribution gap between in-the-wild motions and training data, thereby enhancing generalization capabilities. With the ability to track unseen motions, we also design a set of tuning settings for the RL-TTA strategy, making it possible to restore even diverse and highly difficult motions. 
% \textbf{For Kinematics flaw motions}, 
% % monocular video motion capture algorithms sometimes estimate short-term flawed motions, and directly restoring these motions may lead to failure or collapse. Therefore, 
% we propose a mask-conditioned correction module (MCM) to repair the short-term flawed motions and ensure motion continuity. Guided by the rich shape and motion information provided by the original motion context and segmentation mask,
% % estimated from the original video, 
% we regenerate contextually consistent and reasonable motions to replace the flawed motion, allowing the entire motion sequence to be accurately and fully mapped into the physical space.


To validate the effectiveness of our proposed motion restoration method, we collected 206 high-difficulty motion videos entirely in the wild, including activities such as rhythmic gymnastics, taekwondo, and yoga. These motions exhibit patterns that are significantly more challenging than those in the training set. Our method demonstrated strong performance on this in-the-wild test set, further proving the effectiveness of our approach.

% The resulting simulated motions reinforce physical constraints and eliminate artifacts such as floating, foot sliding, self-penetration, and ground penetration. However, 

% While reinforcement learning methods have shown good performance in simulating locomotion tasks for human motion, they often suffer from poor generalization. For example, simulators that can effectively replicate dance data tend to fail when applied to martial arts sequences. \lrh{move this to paragraph 4.}
% This presents a challenge in developing a physical restore model for diverse motions. 


% to track high-difficult motions, is also adopted in

% The trial-and-error nature of reinforcement learning suggests the possibility of test-time adaptation without the need for additional manual annotations. Therefore, we propose a reinforcement learning-based test-time adaptation strategy (RL-TTA), which allows our physical transfer module to target adjustments to specific motion types or sequences during testing, 
% it  and . making it possible to restore diverse and difficult motions.   with a set of tuning settings
% This approach enhances the generalization capability of the motion refinement model.

% This is due to the strong dependence of the motion refinement method on the reference motion. The refinement process's reliance on physical realism places higher demands on the robustness of motion generation methods. 
% However, current video motion capture methods still experience brief breakdowns and inconsistencies during occlusions or complex movements. 
% Although these issues may not be easily reflected in evaluation metrics, short-term flawed motions can severely affect motion quality, making it difficult for physical simulation to succeed.
Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose a plug-and-play motion restoration method that enhances the physical realism of motions captured from monocular video. Our method can be integrated with state-of-the-art motion capture algorithms to improve the efficiency of obtaining high-quality 3D motion.
    % \item We propose a novel captured motion restoration task that aims to design a plug-and-play method to optimize the physical plausibility of diverse motions obtained from evolving video motion capture techniques.

    \item We introduced an MCM for correcting short-term flawed motions, producing consistent and imitation-friendly motions for physical restoration.
    
    \item We introduced an RL-TTA strategy that allows the physical restoration of high-difficulty in-the-wild motions. We addresses the ``last mile" issue for deploying monocular motion capture algorithms, enabling it to become a viable solution for obtaining high-quality 3D motion.
    
   
    \item We collect 206 videos with high-difficulty in-the-wild motions for testing the generalization of video motion capture methods. Also, we provide a comprehensive benchmark for the task and demonstrate the evaluation of our method across multiple datasets, results show the effectiveness of our method.
    % To showcase the strength of our model, we conduct experiments on widely adopted \textsc{Volleyball} and \textsc{Collective Activity} datasets. The results demonstrate that our method achieves state-of-the-art performance. % using only the keypoints modality. 
\end{itemize} 




% \definecolor{darkblue}{RGB}{52,121,184}
% \definecolor{lightblue}{RGB}{206,230,255}
% \definecolor{midblue}{RGB}{165,189,225}
% \begin{figure}[t]
% \begin{minipage}{\columnwidth}
% \scalebox{0.8}{
% \includegraphics[width=\columnwidth]{picture/tesres.png}
% }
% \end{minipage}
% \begin{minipage}{\columnwidth}
% \scalebox{0.85}{
% \begin{tabular}{lcccccc}
% \arrayrulecolor{darkblue}
% \toprule[1.5pt]
% F-statistics $\uparrow$ & t=5  & t=6 & t=7 & t=8 & t=9 & t=10\\
% \midrule
% $\mathcal{R \rightarrow I}$ & 1.055 & 1.070 & \textbf{1.092} & 1.069 & 1.045 & 1.060\\
% $\mathcal{I \rightarrow R}$ & 1.067 & \textbf{1.087} & 1.069 & 1.043 & 1.052 &1.052\\
% \arrayrulecolor{midblue}
% \midrule[1.5pt]
%  $\alpha$ & 0.150 & 0.100 & 0.050 & 0.020  & 0.010 & 0.005  \\
% F-Critical & 1.041 & 1.052 & 1.066 & 1.084  & 1.095 & 1.106 \\
% \rowcolor{lightblue}
% Confidence & 85\% & 90\% & 95\% & 98\%  & 99\% & 99.5\% \\
% \arrayrulecolor{darkblue}
% % \hline
% \bottomrule[1.5pt]
% \end{tabular}
% }
% \end{minipage}
% \caption{\textbf{The confidence in the bidirectional causality.}
% F-Critical shows the F-Critical Value at Significance Level $\alpha$. Both $\mathcal{R \rightarrow I}$ and $\mathcal{I \rightarrow R}$ are F-statistics that reflect the confidence in causality. When the F-statistics is greater than the F-Critical Value, we consider it as having a corresponding confidence level that causality exists. $t$ denotes the sequence window for inference. 
% \vspace{-3mm}
% \label{table:statistic}
% }

% \end{figure}



==> backup/intro_1107.tex <==
\section{Introduction}
\label{sec:intro}

Physical plausible 3D human motion is in high demand across various fields, including virtual reality, game, animation industries, and academic research on virtual humans and robotics \cite{colombel2020physically,erickson2020assistive,mehta2017vnect}. With technological advancements, monocular video-based motion capture algorithms provide a fast and convenient pipeline for obtaining kinematically accurate motion \cite{wang2024tram,shen2024world,shin2024wham}. 
However, these methods inherently lack dynamic modeling, resulting in significant physical unrealisms such as floating, foot sliding, self-intersections, and ground penetration.

To enhance physical realism, some methods introduce carefully designed kinematic constraints \cite{zanfir2018monocular,zhang2021learning,zhang2020perceiving,huang2022capturing}, such as adding motion smoothing loss to address jitter and foot optimization loss to mitigate foot sliding and ground penetration. These methods require meticulous tuning of the weights for different loss functions and, fundamentally, do not account for the dynamic characteristics of motion, thus failing to fully resolve the physical realism problem.
Other approaches construct a dynamic model of the human body and then train a network to predict the physical parameters required by the dynamic model \cite{tripathi20233d,li2022d,gartner2022trajectory,xie2021physics}. However, these methods often depend heavily on 3D annotated videos and struggle with generalization, particularly when dealing with complex, high-difficulty motions. Recently, PhysPT \cite{zhang2024physpt} has shown exceptional performance in optimizing standard movements but still lacks an understanding of the distribution and physical principles for complex motions, requiring substantial motion priors for effective operation. However, obtaining realistic data for high-difficulty movements remains a significant challenge.
% heavily on 3D annotated videos and struggle with generalization. 
% \lrh{How does the method based on dynamic model perform in solving the motion quality problems? And what other problems remain?}

Due to the complexity of dynamic models, these approaches often oversimplify dynamic equations, leading to insufficient physical realism. Therefore, to better enhance the physical realism of motion, some methods utilize physically simulated environments and learn motion control strategies within such a virtual physical world to ensure physical realism \cite{yuan2021simpoe,shimada2020physcap,gong2022posetriplet,gartner2022differentiable}. They introduce a motion tracking task: given a reference motion clip, the goal of motion tracking is to reproduce the desired motion in a physically simulated environment.
This approach allows for obtaining physically realistic 3D motions from monocular video in a two-stage process. The first stage uses kinematic methods to estimate pose-accurate motions, while the second stage employs motion tracking as a post-processing model to enhance the physical realism of the motion. This two-stage design effectively avoids the trade-off of modeling both kinematics and dynamics in a single model, demonstrating excellent ability to improve the physical quality of motion. 

% {\color{red}Our goal is to efficiently obtain high-quality, realistic motions while significantly reducing the high costs associated with traditional motion capture.}

Inspired by motion tracking, we aim to design a plug-and-play motion restoration post-processing model to transform motion estimated by monocular video motion capture algorithms into physically realistic motions while preserving consistency with the original video as much as possible. This task is challenging primarily in the following two aspects:
\textbf{(1) Dynamics generalization limits:} Current video motion capture algorithms perform well in wild videos and can capture remarkably high-difficulty motions like backflips and Thomas flares. However, existing motion tracking algorithms require meticulous parameter tuning of the controllers \cite{zhang2024physpt}, which can lead to poor performance in wild motions. Additionally, a single controller struggles to generalize across a diverse range of high-difficulty movements, facing significant catastrophic forgetting issues, where rapid loss of old knowledge occurs when learning new skills \cite{luo2023perpetual}.
\textbf{(2) Kinematics flaw motions:} We observed that motion captured from videos can produce short-term catastrophic errors when estimating challenging movements. Certain flawed motions significantly impact the motion-tracking process, as brief motion breakdowns can easily lead to failure in the simulation.  Moreover, since humans are highly sensitive to short-time discrepancies in motion, this flaw can severely impact motion quality in practical applications.
% , frequently resulting in simulation failures,
% Current motion tracking algorithms struggle to correct complex actions like backflips and Thomas flares. This difficulty arises, on the one hand, due to the complex dynamic characteristics of these motions, which make it challenging to train an effective control strategy for correction; on the other hand, monocular motion capture algorithms often produce catastrophic errors when estimating these challenging actions, further hindering the final output of reasonable motions.

To tackle these challenges, 
we propose a plug-and-play motion restore model that enhances the physical plausibility of motions while faithfully retaining the original movements. 
A physical transfer module is introduced to enhance the physical realism of motion by simulation, along with an RL-based test time adaptation strategy to improve the in-the-wild motion generalization ability and encourage the tracking of high-difficulty motions. Additionally, a mask-conditioned correction module is proposed to handle occasional chaotic frames in the original motion, thereby enhancing the robustness of our restore model.
% Based on motion tracking, we propose a physical transfer module to enhance the physical realism of motion and design additional training strategies and reward functions to improve the tracking of complex actions. Additionally, we introduce an RL-based test time adaptation strategy to improve generalization, along with a mask-based correction module to handle occasional chaotic frames in the given motion, thereby enhancing robustness.


% Additionally, we are committed to providing a more cost-effective and efficient solution for motion capture by building on current video motion capture techniques. 
% Our goal is to quickly obtain high-quality, realistic motions while significantly reducing the high costs associated with traditional motion capture.

\textbf{For physical motion restoration}, the physical transfer module (PTM) is responsible for applying physical constraints to the original motions with a physics simulator.
Specifically, using both large-scale video motion capture data and precise mocap data, we trained a powerful motion-tracking policy that controls the character agent in the simulator to track physically implausible motion captured from video. 
This pre-trained module encompasses rich motion priors, enabling it to restore the physical plausibility of noisy motions effectively. 
% However, it still faces challenges when dealing with in-the-wild movements and high-difficulty motions.
\textbf{For Dynamics generalization limits}, 
% {\color{red}the trial-and-error nature of reinforcement learning suggests we envision the potential for test-time adaptation without the need for additional manual annotations. Consequently}
we propose a reinforcement learning-based test-time adaptation strategy (RL-TTA) that enables targeted adjustments during testing for specific action classes or segments. This strategy can effectively bridge the distribution gap between in-the-wild motions and training data, thereby enhancing generalization capabilities. With the ability to track unseen motions, we also design a set of tuning settings for the RL-TTA strategy, making it possible to restore even diverse and highly difficult motions. 
\textbf{For Kinematics flaw motions}, 
% monocular video motion capture algorithms sometimes estimate short-term flawed motions, and directly restoring these motions may lead to failure or collapse. Therefore, 
we propose a mask-conditioned correction module (MCM) to repair the short-term flawed motions and ensure motion continuity. Guided by the rich shape and motion information provided by the original motion context and segmentation mask,
% estimated from the original video, 
we regenerate contextually consistent and reasonable motions to replace the flawed motion, allowing the entire motion sequence to be accurately and fully mapped into the physical space.

To validate the effectiveness of our proposed motion restoration method, we collected 206 high-difficulty motion videos entirely in the wild, including activities such as rhythmic gymnastics, taekwondo, and yoga. These motions exhibit patterns that are significantly more challenging than those in the training set. Our method demonstrated strong performance on this in-the-wild test set, further proving the effectiveness of our approach.

% The resulting simulated motions reinforce physical constraints and eliminate artifacts such as floating, foot sliding, self-penetration, and ground penetration. However, 

% While reinforcement learning methods have shown good performance in simulating locomotion tasks for human motion, they often suffer from poor generalization. For example, simulators that can effectively replicate dance data tend to fail when applied to martial arts sequences. \lrh{move this to paragraph 4.}
% This presents a challenge in developing a physical restore model for diverse motions. 


% to track high-difficult motions, is also adopted in

% The trial-and-error nature of reinforcement learning suggests the possibility of test-time adaptation without the need for additional manual annotations. Therefore, we propose a reinforcement learning-based test-time adaptation strategy (RL-TTA), which allows our physical transfer module to target adjustments to specific motion types or sequences during testing, 
% it  and . making it possible to restore diverse and difficult motions.   with a set of tuning settings
% This approach enhances the generalization capability of the motion refinement model.

% This is due to the strong dependence of the motion refinement method on the reference motion. The refinement process's reliance on physical realism places higher demands on the robustness of motion generation methods. 
% However, current video motion capture methods still experience brief breakdowns and inconsistencies during occlusions or complex movements. 
% Although these issues may not be easily reflected in evaluation metrics, short-term flawed motions can severely affect motion quality, making it difficult for physical simulation to succeed.
Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose a plug-and-play motion restoration method that enhances the physical realism of motions captured from monocular video. Our method can be integrated with state-of-the-art motion capture algorithms to improve the efficiency of obtaining high-quality 3D motion.
    % \item We propose a novel captured motion restoration task that aims to design a plug-and-play method to optimize the physical plausibility of diverse motions obtained from evolving video motion capture techniques.
    
    \item We introduced an RL-TTA strategy that allows the restoration of high-difficulty motions from in-the-wild videos, and an MCM for correcting short-term flawed motions. Our method addresses the ``last mile" issue for deploying monocular motion capture algorithms, enabling it to become a viable solution for obtaining high-quality 3D motion.
   
    \item We provided a comprehensive benchmark for the task and demonstrated the evaluation of our method across multiple datasets and high-difficulty in-the-wild videos, results show the effectiveness of our method.
    % To showcase the strength of our model, we conduct experiments on widely adopted \textsc{Volleyball} and \textsc{Collective Activity} datasets. The results demonstrate that our method achieves state-of-the-art performance. % using only the keypoints modality. 
\end{itemize} 




% \definecolor{darkblue}{RGB}{52,121,184}
% \definecolor{lightblue}{RGB}{206,230,255}
% \definecolor{midblue}{RGB}{165,189,225}
% \begin{figure}[t]
% \begin{minipage}{\columnwidth}
% \scalebox{0.8}{
% \includegraphics[width=\columnwidth]{picture/tesres.png}
% }
% \end{minipage}
% \begin{minipage}{\columnwidth}
% \scalebox{0.85}{
% \begin{tabular}{lcccccc}
% \arrayrulecolor{darkblue}
% \toprule[1.5pt]
% F-statistics $\uparrow$ & t=5  & t=6 & t=7 & t=8 & t=9 & t=10\\
% \midrule
% $\mathcal{R \rightarrow I}$ & 1.055 & 1.070 & \textbf{1.092} & 1.069 & 1.045 & 1.060\\
% $\mathcal{I \rightarrow R}$ & 1.067 & \textbf{1.087} & 1.069 & 1.043 & 1.052 &1.052\\
% \arrayrulecolor{midblue}
% \midrule[1.5pt]
%  $\alpha$ & 0.150 & 0.100 & 0.050 & 0.020  & 0.010 & 0.005  \\
% F-Critical & 1.041 & 1.052 & 1.066 & 1.084  & 1.095 & 1.106 \\
% \rowcolor{lightblue}
% Confidence & 85\% & 90\% & 95\% & 98\%  & 99\% & 99.5\% \\
% \arrayrulecolor{darkblue}
% % \hline
% \bottomrule[1.5pt]
% \end{tabular}
% }
% \end{minipage}
% \caption{\textbf{The confidence in the bidirectional causality.}
% F-Critical shows the F-Critical Value at Significance Level $\alpha$. Both $\mathcal{R \rightarrow I}$ and $\mathcal{I \rightarrow R}$ are F-statistics that reflect the confidence in causality. When the F-statistics is greater than the F-Critical Value, we consider it as having a corresponding confidence level that causality exists. $t$ denotes the sequence window for inference. 
% \vspace{-3mm}
% \label{table:statistic}
% }

% \end{figure}



==> backup/method_1108.tex <==
\section{Physics-based Motion Restoration}
Our method takes video-captured motion as reference motions and focuses on restoring their physical realism while preserving the original patterns of the reference motions. The final output is restored motion. We define reference motions as ${x}_t$, which consists of the joints position ${p}_t \in \mathbb{R}^{J \times 3}$ and the joints 6-dim rotation $\mathcal{\theta}_t \in \mathbb{R}^{J \times 6}$ \cite{zhou2019continuity} (compatible with SMPL format). $J$ means the joint number of the humanoid.
We also take reference velocities ${q}_t$ as input, which consists of the linear velocity ${v}_t \in \mathbb{R}^{J \times 3}$ and angular ${w}_t \in \mathbb{R}^{J \times 6}$ velocity. 
An overview of our method is provided in Fig \ref{fig:pipeline}. When a mismatch between the reference motion and segmentation mask is detected, our MCM is performed to correct the flawed motion. After that, a pre-trained PTM transfers the original motion into physical space. Since it's highly difficulty to track complex and in-the-wild motions, the transfer process often fails and calls for the RL-TTA strategy to specifically adapt the motion instance until success or meets the step threshold.

% In Section 3.1, we introduce the physics-based motion transfer module. In Section 3.2, we provide detailed explanations of the RL-TTA strategy. Finally, we briefly describe the inbetweening module in Section 3.3.
% (special settings) and how it is applied to in-the-wild motions, which are more challenging than those found in the training set.

\subsection{Physics-based Motion Transfer Module\zyc{See LaTeX comments}} %这部分的写法看不出那部分是咱们新提出来的。可以考虑增加：为解决其中什么子问题，提出了什么。
The problem of controlling a humanoid to follow a reference motion sequence $q_{b_{1:T}}$ can be formulated as a Markov Decision Process (MDP), defined by the tuple $M = \langle S, A, P_{\text{physics}}, R, \gamma \rangle$, which consists of states, actions, transition dynamics, reward function, and a discount factor. 
The physics simulator provides the state $S$, reward $R$, and transition dynamics $P$, while the policy $\pi_{\text{PMT}}$ determines the action $A$. At each time step $t$, the agent selects an action $a_t$ from the policy $\pi_{\text{PMT}}(a_t|s_t)$ based on the current state $s_t$, and the environment responds with the next state $s_{t+1}$ and a reward $r_t$. Proximal Policy Optimization (PPO) \cite{schulman2017proximal} is used to optimize the policy $\pi^*_{\text{PMT}}$ to maximize the expected discounted return $\mathbb{E}\left[\sum_{t=1}^{T}\gamma^{t-1}r_{t}\right]$.

\textbf{States.} The state $s_{t}$ consists of the physical state of the humanoid ${x}_t$ (including positions, rotations, and linear and angular velocities of the humanoid) as well as the next frame information ${g}_t$ from the ref motion.  We define ${g}_t$ as the difference between the next time step reference motion and the current frame humanoid state.
% (use rotation difference for $\mathcal{\theta}_t$). 
Unlike directly using the next frame of the reference motion, leveraging the difference between the current and reference frames has been shown to effectively inform the policy on compensating for the pose residual \cite{yuan2023physdiff}.

\textbf{Action.} The action $a_t$ specifies the target joint angles for the Proportional-Derivative (PD) controller at each degree of freedom (DoF) of the humanoid joints.
Given an action, the torque to be applied is computed as:
\begin{equation}
\tau^i=k_p^i(a_t^i-x_t^i)-k_d^iq_t^i ,
\end{equation}
where $i$ means joint DoF index, $k_p$ and $k_d$ are manually-specified gains. This design helps our method perform better when the reference motion is unreal and noisy \cite{luo2023perpetual}. 
% since our controller is designed to handle repair task.

\textbf{Policy.} The policy $\pi_{\text{PTM}}$ is represented by a Gaussian distribution with a fixed diagonal covariance matrix. Our policy utilizes a neural network map state $s_t$ to the mean $\nu_t$ of the distribution. Our network is constructed with 6-layer multilayer perceptions and ReLU activation functions. A discriminator, with the same observations, loss function, and gradient penalty as AMP \cite{peng2021amp}, is used to predict whether a given state $s_t$ and action $a_t$ is sampled from the demonstrations $M$ or generated by policy $\pi_{\text{PTM}}$. 
% Our discriminator is an MLP with two hidden layers with ReLU activation function.


\subsection{RL-based Test Time Adaptation}
% Current video motion capture methods can generate surprisingly complex motions, particularly in in-the-wild videos. 
% However, it remains highly challenging to project these motions into the physical space through post-processing motion restoration.
% Due to the inherent generalization limitations of reinforcement learning, a purely PTM still struggles to handle in-the-wild motions. 
% This approach enables the repair of physical realism in high-difficulty in the wild motions.
With the success of motion tracking on large-scale motion datasets, the availability of rich motion priors opens up the possibility for rapid adaptation during test time. Therefore, we propose the RL-TTA, which involves performing a limited number of experiment steps on the current test data under specific adaptation settings (updating network parameters). 
In addition to the challenges of generalization, high-difficulty motions differ from locomotion tasks in several key ways:
1) Complex airborne poses.
2) Rapidly shifting root positions.
3) Extreme body postures.
Our method addresses these issues through the following design.

\textbf{Relative Reward.}
% To ensure accurate reproduction of the reference motion, the motion simulation strategy
% Motion tracking methods typically construct a multi-dimensional reward to encourage the model to align closely with the reference, which usually includes position, rotation, velocity, and angular velocity. 
% guide the humanoid’s reconstruction from various perspectives, 
% These components imposing strong constraints on the motion simulation, which trap the model in the minutiae of reconstruction, slowing or even stalling the overall tracking process.
% . However, such strict constraints can
% In physical motion restoration tasks, 
 %, making it hard to follow.
% meaning we don't need to fully follow the reference motion. 
The captured reference motion contains error-accumulating roots and jitter poses that need to be repaired, making it detrimental to construct a full reconstruction reward.
Therefore, we designed a relative reward that neglects the absolute root position of the rigid body, maintaining global orientation and translation information through explicit guidance from rotation and implicit guidance from velocity. The relative reward is formulated as: \zyc{what's$\ominus$?}
\begin{equation}\begin{aligned}&r_{t}^{\mathrm{g}}=w_{\mathrm{p}}e^{-100\|rela(\boldsymbol{\hat{p}}_{t})-rela(\boldsymbol{p}_{t})\|}+w_{\mathrm{r}}e^{-10\|\boldsymbol{\hat{\theta}}_{t}\ominus\boldsymbol{\theta}_{t}\|}\\&+w_{\mathrm{v}}e^{-0.1\|\boldsymbol{\hat{v}}_{t}-\boldsymbol{v}_{t}\|}+w_{\mathrm{\omega}}e^{-0.1\|\boldsymbol{\hat{\omega}}_{t}-\boldsymbol{\omega}_{t}\|},\end{aligned}\end{equation}
where $\boldsymbol{\hat{p}}_{t}$ means the joint position of reference motion, $rela()$ means to ignore the gravity axis part of root joints.
The overall reward is defined as the sum of tracking reward $r_t^\mathrm{g}$, style reward $r_t^\mathrm{amp}$, and energy penalty $r_t^\mathrm{energy}$ \cite{peng2018deepmimic}:
\begin{equation}r_t=0.5r_t^\mathrm{g}+0.5r_t^\mathrm{amp}+r_t^\mathrm{energy}.\end{equation}
% allowing the model to restore the motion while disregarding unreasonable root movement and jitter. The humanoid's global orientation and displacement are maintained through explicit guidance from rotation and implicit guidance from velocity.


% To improve training efficiency and prevent undesirable behaviors or unstable states, early termination is often employed during policy training. The distance termination condition proposed in UHC performs well in many tasks. However, in high-difficulty motion simulations, frequent floating and aerial movements often prematurely trigger distance termination.
% Therefore, we modified the distance termination based on relative position and introduced early termination conditions based on joint height and ground contact, ensuring its applicability to complex motions while preserving its advantages. The relative position adjustment reduces sensitivity to floating and jitter, allowing the model to focus more on the motion itself. The ground contact condition further refines failure boundaries in ground interactions, which are critical for high-difficulty motions involving complex ground interactions, such as yoga and breakdancing.

% Since high-difficulty reference motion often involves frequent floating and aerial movements, making the displacement between humanoid
\textbf{Early Termination.} In high-difficulty motion tracking, there is a large displacement between humanoid and reference motion, as reference motion often involves frequent floating and aerial movements. This phenomenon makes defining when an experiment should be terminated challenging, which is crucial for training efficiency and preventing undesirable behaviors. Therefore, we design a relative termination condition by calculating each joint's mean relative distance between humanoid and reference motion.
% , assuming their roots coincide at a single point. 
Experiments will be terminated when the distance is larger than threshold $d$. We also introduce termination condition $\mathcal{F}^h_t$ and $\mathcal{F}^c_t$ based on joint height and ground contact to end the experiments when falls and erroneous contacts occur. The full termination $\mathcal{F}_t$ is formulated as:
\begin{equation}
    \mathcal{F}_t = \left( \frac{1}{J} \sum_{i=1}^{J} \|rela(\boldsymbol{\hat{p}}^{i}_{t})-rela(\boldsymbol{p}^{i}_{t})\| > d \right) \vee \mathcal{F}^h_t \vee \mathcal{F}^c_t
\end{equation} 

\zyc{How to get the threshold $d$? } %这个阈值的设定是根据什么设计的，不同数据之间是否有差异？

\textbf{Residual Force.} During the test-time adaptation phase, we introduce residual forces \cite{yuan2020residual} to compensate for the dynamics mismatch.
% and more effectively imitate the reference motion. 
This is important because complex motions often involve airborne flips and jumps (commonly seen in gymnastics and martial arts), which frequently rely on elastic trampolines and mats for execution. The use of external forces is necessary to account for the absence of these environmental conditions in our simulations.
% Since the motion restoration scenarios involve a wider variety of force application points (e.g., hand support in handstands, waist control in backflips, and footwork in ballet), we define residual forces on all joints of the humanoid. 
% Additionally, we relax the regularization constraints on these external forces to allow for greater flexibility in addressing the specific force requirements of different motions.

\textbf{Test-Time Adaptation.} In practical applications, our test-time adaptation approach can be implemented in two distinct forms. The first is Source-Free Domain Adaptation, which involves adapting our model within a certain amount of data,
% randomly sampling data prior to testing for domain fitting, 
allowing the capabilities of the model can be transferred across the entire dataset. This approach is suitable for optimizing low-difficulty motions within specific subdomains.
The second form is Test-Time Instance Adaptation, where each motion sequence is treated as an individual instance, and the adaptation is performed for each instance independently. This method is particularly useful when dealing with high-difficulty motions or when the reference motion data is of low quality.

\subsection{Mask-conditioned Motion Correction Module}
Through our PTM and RL-TTA strategy, we have successfully enhanced the physical realism of many high-difficulty motions. However, in practice, we observed that current video motion capture methods still struggle with temporary breakdowns when dealing with complex motions. These breakdowns manifest as incoherent frames within the motion sequence that are inconsistent with the surrounding context. Although such brief disruptions have a minimal impact on overall metrics, they can easily cause failures in the physics simulation process and are obvious in the human senses.
To address this issue, we propose a mask-conditioned in-betweening module. This module replaces the broken frames with smooth motions, leveraging the contextual information from the reference motion and mask data derived from segmentation.

\textbf{Mismatch Detection.} 
Given the reference motion and its corresponding video, we project the absolute 3D positions of the reference motion into 2D camera coordinates. We then use an object detection algorithm to extract the corresponding 2D keypoints from the video. Using the Object Keypoint Similarity (OKS) algorithm, we compute the matching degree between the two sets of keypoints and obtain a similarity score sequence. Frames with a similarity score below a certain threshold will be flagged as containing poor-quality motions. \zyc{what the symbols are? is d the threshold?}
\begin{equation}OKS=\frac{\sum_iexp(-d_i^2/2s^2\sigma_i^2)\delta(v_i>0)}{\sum_i\delta(v_i>0)}\end{equation}
Additionally, segmentation algorithms can also be used to detect poor-quality motions. We project the SMPL-generated mesh onto the 2D plane and treat it as a set of pixel points. 
The matching similarity can be calculated by determining the proportion of projected mesh points that are contained within the human mask.
% The matching similarity can be determined by calculating the Intersection over Union (IoU) similarity between the segmented mask set and the projected mesh set.

\textbf{Motion Representation.} \zyc{See the latex comments here!}%这部分和下一部分没有写清楚，Motion Representation 是创新吗？不是的话简洁些，是的话这个表示创新在哪里？有啥好处没有写清楚； Mask-conditioned Motion Diffusion In-betweening这里写的不是很好，重点放在训练任务的设计上，为扩散模型设计了什么训练任务，为了达到这一目标对输入的条件进行了哪些操作，目前写的只是怎么做，没有很好突出任务的设计。
Given a human motion sequence $x \in \mathbb{R}^{N \times D}$, the segmented human mask $m \in \mathbb{R}^{N \times w \times h}$, and a keyframe signal (which identifies frames requiring inbetweening), this module restore the mismatched motion frames. The human motion $x$ is derived from the reference motion, where we compute a 135-dimensional motion representation based on SMPL parameters, which includes 3-dim translation, 6-dim root rotation, and 21 body joint rotations.
The observation signal is generated from the mismatch detection algorithm.

\textbf{Mask-conditioned Diffusion In-betweening.} 
Before executing the diffusion model \cite{karunratanakul2023gmd,cohan2024flexible}, we use a Vision Transformer (ViT) \cite{alexey2020image} to extract human pose and shape features from the human mask. The extracted low-dimensional features are used as the mask condition for the diffusion process. 
Only the motion frames that need to be replaced should be subjected to noise, while the remaining parts are retained as the motion context.
To inform the model which frame can be observed, we also concatenate the resulting masked sample $x_t$ with the keyframe signal as input to the diffusion model. The image mask features are combined similarly, ensuring that both the temporal keyframes and spatial mask features guide the diffusion process effectively. 

\textbf{Motion Correction Goal Design}
Unlike traditional inbetween methods, the goal of the MCM is to replace flawed motions in the reference sequence based on contextual information, ensuring that the corrected reference motion is smooth and continuous. Thus, we focus solely on the model’s ability to fill temporal gaps. Given that the input to the MCM is motion captured from video, it is crucial to ensure that the generated motion remains as consistent as possible with the original video content. To achieve this, we use the human mask obtained from segmentation as a conditional signal to guide the inbetween process.

\textbf{Training process}
We use motion captured from videos as the training data. A random segment of motion, selected at a random position within the entire motion sequence, is chosen as the generation target. Both keyframe conditioning signals $c$ and mask conditioning signal $m$ are set to $\emptyset$ for 10\% of training samples to make our model suited for unconditioned motion generation.




==> backup/method_1110.tex <==
\section{Physics-based Motion Restoration}
Our method takes video-captured motion as reference motions and focuses on restoring their physical realism while preserving the original patterns of the reference motions. The final output is restored motion. We define reference motions as ${x}_t$, which consists of the joints position ${p}_t \in \mathbb{R}^{J \times 3}$ and the joints 6-dim rotation $\mathcal{\theta}_t \in \mathbb{R}^{J \times 6}$ \cite{zhou2019continuity} (compatible with SMPL format). $J$ means the joint number of the humanoid.
We also take reference velocities ${q}_t$ as input, which consists of the linear velocity ${v}_t \in \mathbb{R}^{J \times 3}$ and angular ${w}_t \in \mathbb{R}^{J \times 6}$ velocity. 
An overview of our method is provided in Fig \ref{fig:pipeline}. When a mismatch between the reference motion and segmentation mask is detected, our MCM is performed to correct the flawed motion. After that, a pre-trained PTM transfers the original motion into physical space. Since it's highly difficulty to track complex and in-the-wild motions, the transfer process often fails and calls for the RL-TTA strategy to specifically adapt the motion instance until success or meets the step threshold. 

% In Section 3.1, we introduce the physics-based motion transfer module. In Section 3.2, we provide detailed explanations of the RL-TTA strategy. Finally, we briefly describe the inbetweening module in Section 3.3.
% (special settings) and how it is applied to in-the-wild motions, which are more challenging than those found in the training set.

\subsection{Mask-conditioned Motion Correction Module}
% Through our PTM and RL-TTA strategy, we have successfully enhanced the physical realism of many high-difficulty motions. However, in practice, we observed that current video motion capture methods still struggle with temporary breakdowns when dealing with complex motions. 
Flaw motions in video capture results manifest as incoherent frames within the motion sequence inconsistent with the surrounding motion context. Although such brief disruptions have a minimal impact on metrics, they can easily cause failures in the physics simulation process and are obvious in the human senses.
To address this issue, our MCM first detects flawed motion, then regenerates the problematic motion segment guided by the motion context and human mask signals, ultimately replacing the flawed motion.
% we replace the broken frames with smooth motions, leveraging the contextual information from the reference motion and mask data derived from segmentation.

\textbf{Mismatch Detection.} 
Given the reference motion and its corresponding video, we project the 3D positions of the reference motion into 2D camera coordinates. Also, an object detection algorithm is used to extract the corresponding 2D keypoints from the video. Using the Object Keypoint Similarity (OKS) algorithm, we compute the matching degree between the two sets of keypoints and obtain a similarity score sequence. Frames with a similarity score below a certain threshold will be flagged as flaw motion. 
% \zyc{what the symbols are? is d the threshold?}
\begin{equation}OKS=\frac{\sum_iexp(-d_i^2/2s^2)\delta(v_i>0)}{\sum_i\delta(v_i>0)}\end{equation}
where $v_i$ represents the visibility flag, $s_i$ denotes the scale factor, and $d_i$ is the distance difference between the projection and the detection results.
Additionally, segmentation algorithms can also be used to detect flaw motion. We project the SMPL-generated mesh onto the 2D plane and treat it as a set of pixel points. 
The matching similarity can be calculated by determining the proportion of projected mesh points that are contained within the human mask.
% The matching similarity can be determined by calculating the Intersection over Union (IoU) similarity between the segmented mask set and the projected mesh set.

% \textbf{Motion Representation.} \zyc{See the latex comments here!}%这部分和下一部分没有写清楚，Motion Representation 是创新吗？不是的话简洁些，是的话这个表示创新在哪里？有啥好处没有写清楚； Mask-conditioned Motion Diffusion In-betweening这里写的不是很好，重点放在训练任务的设计上，为扩散模型设计了什么训练任务，为了达到这一目标对输入的条件进行了哪些操作，目前写的只是怎么做，没有很好突出任务的设计。
% Given a human motion sequence $x \in \mathbb{R}^{N \times D}$, the segmented human mask $m \in \mathbb{R}^{N \times w \times h}$, and a keyframe signal (which identifies frames requiring inbetweening), this module restore the mismatched motion frames. The human motion $x$ is derived from the reference motion, where we compute a 135-dimensional motion representation based on SMPL parameters, which includes 3-dim translation, 6-dim root rotation, and 21 body joint rotations.
% The observation signal is generated from the mismatch detection algorithm.

\textbf{Motion Correction Goal Design.}
Unlike traditional inbetween methods, the goal of the MCM is to replace flawed motions in the reference sequence based on contextual information, ensuring that the corrected reference motion is smooth and continuous. Thus, we focus solely on the model’s ability to fill temporal gaps. Given that the input to the MCM is motion captured from video, it is crucial to ensure that the generated motion remains as consistent as possible with the original video content. To achieve this, we use the human mask obtained from segmentation as a conditional signal to guide the inbetween process.

\textbf{Mask-conditioned Diffusion In-betweening.} 
Given a reference motion sequence $x \in \mathbb{R}^{N \times D}$, the segmented human mask $m \in \mathbb{R}^{N \times w \times h}$, and a keyframe signal (generated from the mismatch detection, identifies frames requiring correction), this module correct the reference motion by replacing mismatched motion frames.
% Before executing the diffusion model \cite{karunratanakul2023gmd,cohan2024flexible}, we use a Vision Transformer (ViT) \cite{alexey2020image} to extract human pose and shape features from the human mask. 
We employ a pre-trained Vision Transformer (ViT) as the mask feature extractor to capture rich human pose information from the segmentation mask.
The extracted features are used as the mask condition for the diffusion process. 
% Only the motion frames that need to be replaced should be subjected to noise, while the remaining parts are retained as the motion context.
% To inform the model which frame can be observed, we also concatenate the resulting sample $x_t$ with the keyframe signal as input to the diffusion model. The image mask features are combined similarly, ensuring that both the temporal keyframes and spatial mask features guide the diffusion process effectively. 
Following \cite{karunratanakul2023gmd,cohan2024flexible}, we concatenate the resulting sample $x_t$, keyframe signal and mask features as model input to inform the generation model with condition signal.

\textbf{Training process.}
We use motion captured from videos as the training data. A random segment of motion, selected at a random position within the entire motion sequence, is chosen as the generation target. Our model is trained to reconstruct this segment. Both keyframe conditioning signals $c$ and mask conditioning signal $m$ are set to $\emptyset$ for 10\% of training samples to make our model suited for unconditioned motion generation.



\subsection{Physics-based Motion Transfer Module\zyc{See LaTeX comments}} %这部分的写法看不出那部分是咱们新提出来的。可以考虑增加：为解决其中什么子问题，提出了什么。
The problem of controlling a humanoid to follow a reference motion sequence $q_{b_{1:T}}$ can be formulated as a Markov Decision Process (MDP), defined by the tuple $M = \langle S, A, P_{\text{physics}}, R, \gamma \rangle$, which consists of states, actions, transition dynamics, reward function, and a discount factor. 
The physics simulator provides the state $S$, reward $R$, and transition dynamics $P$, while the policy $\pi_{\text{PTM}}$ determines the action $A$. At each time step $t$, the agent selects an action $a_t$ from the policy $\pi_{\text{PTM}}(a_t|s_t)$ based on the current state $s_t$, and the environment responds with the next state $s_{t+1}$ and a reward $r_t$. Proximal Policy Optimization (PPO) \cite{schulman2017proximal} is used to optimize the policy $\pi^*_{\text{PTM}}$ to maximize the expected discounted return $\mathbb{E}\left[\sum_{t=1}^{T}\gamma^{t-1}r_{t}\right]$.

\textbf{States.} The state $s_{t}$ consists of the physical state of the humanoid ${x}_t$ (including positions, rotations, and linear and angular velocities) as well as the next frame information ${g}_t$ from the reference motion.  We define ${g}_t$ as the difference between the next frame reference motion and the current frame humanoid state.
% (use rotation difference for $\mathcal{\theta}_t$). 
Unlike directly using the next frame of the reference motion, leveraging the difference has been shown to effectively inform the policy on compensating for the pose residual \cite{yuan2023physdiff}.

\textbf{Action.} The action $a_t$ specifies the target joint angles for the Proportional-Derivative (PD) controller at each degree of freedom (DoF) of the humanoid joints.
Given an action, the torque to be applied is computed as:
\begin{equation}
\tau^i=k_p^i(a_t^i-x_t^i)-k_d^iq_t^i ,
\end{equation}
where $i$ means joint DoF index, $k_p$ and $k_d$ are manually-specified gains. This design helps our method perform better when the reference motion is unreal and noisy \cite{luo2023perpetual}. 
% since our controller is designed to handle repair task.

\textbf{Policy.} The policy $\pi_{\text{PTM}}$ is represented by a Gaussian distribution with a fixed diagonal covariance matrix. Our policy utilizes a neural network map state $s_t$ to the mean $\nu_t$ of the distribution. Our network is constructed with 6-layer multilayer perceptions and ReLU activation functions. A discriminator, with the same observations, loss function, and gradient penalty as AMP \cite{peng2021amp}, is used to predict whether a given state $s_t$ and action $a_t$ is sampled from the demonstrations $M$ or generated by policy $\pi_{\text{PTM}}$. 
% Our discriminator is an MLP with two hidden layers with ReLU activation function.


\subsection{RL-based Test Time Adaptation}
% Current video motion capture methods can generate surprisingly complex motions, particularly in in-the-wild videos. 
% However, it remains highly challenging to project these motions into the physical space through post-processing motion restoration.
% Due to the inherent generalization limitations of reinforcement learning, a purely PTM still struggles to handle in-the-wild motions. 
% This approach enables the repair of physical realism in high-difficulty in the wild motions.
With the success of motion tracking on large-scale motion datasets, the availability of rich motion priors opens up the possibility for rapid adaptation during test time. Therefore, we propose the RL-TTA, which involves performing a limited number of experiment steps on the current test data under specific adaptation settings (updating network parameters). 
In addition to the challenges of generalization, high-difficulty motions differ from locomotion tasks in several key ways:
1) Complex airborne poses.
2) Rapidly shifting root positions.
3) Extreme body postures.
Our method addresses these issues through the following design.

\textbf{Relative Reward.}
% To ensure accurate reproduction of the reference motion, the motion simulation strategy
% Motion tracking methods typically construct a multi-dimensional reward to encourage the model to align closely with the reference, which usually includes position, rotation, velocity, and angular velocity. 
% guide the humanoid’s reconstruction from various perspectives, 
% These components imposing strong constraints on the motion simulation, which trap the model in the minutiae of reconstruction, slowing or even stalling the overall tracking process.
% . However, such strict constraints can
% In physical motion restoration tasks, 
 %, making it hard to follow.
% meaning we don't need to fully follow the reference motion. 
The captured reference motion contains error-accumulating roots and jitter poses that need to be repaired, making it detrimental to construct a full reconstruction reward.
Therefore, we designed a relative reward that neglects the absolute root position of the rigid body, maintaining global orientation and translation information through explicit guidance from rotation and implicit guidance from velocity. The relative reward is formulated as: 
\begin{equation}\begin{aligned}&r_{t}^{\mathrm{g}}=w_{\mathrm{p}}e^{-100\|rela(\boldsymbol{\hat{p}}_{t})-rela(\boldsymbol{p}_{t})\|}+w_{\mathrm{r}}e^{-10\|\boldsymbol{\hat{\theta}}_{t}\ominus\boldsymbol{\theta}_{t}\|}\\&+w_{\mathrm{v}}e^{-0.1\|\boldsymbol{\hat{v}}_{t}-\boldsymbol{v}_{t}\|}+w_{\mathrm{\omega}}e^{-0.1\|\boldsymbol{\hat{\omega}}_{t}-\boldsymbol{\omega}_{t}\|},\end{aligned}\end{equation}
where $\boldsymbol{\hat{p}}_{t}$ means the joint position of reference motion, $rela()$ means to ignore the gravity axis part of root joints. $\ominus$ means rotation difference.
The overall reward is defined as the sum of tracking reward $r_t^\mathrm{g}$, style reward $r_t^\mathrm{amp}$, and energy penalty $r_t^\mathrm{energy}$ \cite{peng2018deepmimic}:
\begin{equation}r_t=0.5r_t^\mathrm{g}+0.5r_t^\mathrm{amp}+r_t^\mathrm{energy}.\end{equation}
% allowing the model to restore the motion while disregarding unreasonable root movement and jitter. The humanoid's global orientation and displacement are maintained through explicit guidance from rotation and implicit guidance from velocity.


% To improve training efficiency and prevent undesirable behaviors or unstable states, early termination is often employed during policy training. The distance termination condition proposed in UHC performs well in many tasks. However, in high-difficulty motion simulations, frequent floating and aerial movements often prematurely trigger distance termination.
% Therefore, we modified the distance termination based on relative position and introduced early termination conditions based on joint height and ground contact, ensuring its applicability to complex motions while preserving its advantages. The relative position adjustment reduces sensitivity to floating and jitter, allowing the model to focus more on the motion itself. The ground contact condition further refines failure boundaries in ground interactions, which are critical for high-difficulty motions involving complex ground interactions, such as yoga and breakdancing.

% Since high-difficulty reference motion often involves frequent floating and aerial movements, making the displacement between humanoid
\textbf{Early Termination.} In high-difficulty motion tracking, there is a large displacement between humanoid and reference motion, as reference motion often involves frequent floating and penetration. This phenomenon makes defining when an experiment should be terminated challenging, which is crucial for training efficiency and preventing undesirable behaviors. Therefore, we design a relative termination condition by calculating each joint's mean relative distance between humanoid and reference motion.
% , assuming their roots coincide at a single point. 
Experiments will be terminated when the distance is larger than threshold $d$. We also introduce termination condition $\mathcal{F}^h_t$ and $\mathcal{F}^c_t$ based on joint height and ground contact to end the experiments when falls and erroneous contacts occur. The full termination $\mathcal{F}_t$ is defined below, with a smaller threshold $d$ indicating a stricter adherence to the reference motion.
\begin{equation}
    \mathcal{F}_t = \left( \frac{1}{J} \sum_{i=1}^{J} \|rela(\boldsymbol{\hat{p}}^{i}_{t})-rela(\boldsymbol{p}^{i}_{t})\| > d \right) \vee \mathcal{F}^h_t \vee \mathcal{F}^c_t
\end{equation} 
 

% \zyc{How to get the threshold $d$? } %这个阈值的设定是根据什么设计的，不同数据之间是否有差异？

\textbf{Residual Force.} During the test-time adaptation phase, we introduce residual forces \cite{yuan2020residual} to compensate for the dynamics mismatch.
% and more effectively imitate the reference motion. 
This is important because complex motions often involve airborne flips and jumps (commonly seen in gymnastics and martial arts), which frequently rely on elastic trampolines and mats for execution. The use of external forces is necessary to account for the absence of these environmental conditions in our simulations.
% Since the motion restoration scenarios involve a wider variety of force application points (e.g., hand support in handstands, waist control in backflips, and footwork in ballet), we define residual forces on all joints of the humanoid. 
% Additionally, we relax the regularization constraints on these external forces to allow for greater flexibility in addressing the specific force requirements of different motions.

\textbf{Test-Time Adaptation.} In practical applications, our test-time adaptation approach can be implemented in two distinct forms. The first is Source-Free Domain Adaptation, which involves adapting our model within a certain amount of data,
% randomly sampling data prior to testing for domain fitting, 
allowing the model's capabilities to be transferred across the entire dataset. This approach is suitable for optimizing low-difficulty motions within specific subdomains.
The second form is Test-Time Instance Adaptation, where each motion sequence is treated as an individual instance, and the adaptation is performed for each instance independently. This method is particularly useful when dealing with high-difficulty and low quality motions.
% when the reference motion data is of low quality.






==> backup/method_1112.tex <==
\section{Physics-based Motion Restoration}
Our method takes video-captured motion as reference motions and focuses on restoring their physical realism while preserving the original patterns of the reference motions. The final output is restored motion. We define reference motions as ${x}_t$, which consists of the joints position ${p}_t \in \mathbb{R}^{J \times 3}$ and the joints 6-dim rotation $\mathcal{\theta}_t \in \mathbb{R}^{J \times 6}$ \cite{zhou2019continuity} (compatible with SMPL format). $J$ means the joint number of the humanoid.
We also take reference velocities ${q}_t$ as input, which consists of the linear velocity ${v}_t \in \mathbb{R}^{J \times 3}$ and angular ${w}_t \in \mathbb{R}^{J \times 6}$ velocity. 
An overview of our method is provided in Fig \ref{fig:pipeline}. When a mismatch between the reference motion and segmentation mask is detected, our MCM is performed to correct the flawed motion. After that, our PTM transfers the original motion into physical space. Since it's difficult to track complex and in-the-wild motions, the transfer process often fails and starts specifically adapting current motion until success or meets the step threshold. 

% In Section 3.1, we introduce the physics-based motion transfer module. In Section 3.2, we provide detailed explanations of the RL-TTA strategy. Finally, we briefly describe the inbetweening module in Section 3.3.
% (special settings) and how it is applied to in-the-wild motions, which are more challenging than those found in the training set.

\subsection{Mask-conditioned Motion Correction Module}
% Through our PTM and RL-TTA strategy, we have successfully enhanced the physical realism of many high-difficulty motions. However, in practice, we observed that current video motion capture methods still struggle with temporary breakdowns when dealing with complex motions. 
Flaw motions in video capture results manifest as incoherent frames within the motion sequence inconsistent with the surrounding motion context. Although such brief disruptions have a minimal impact on metrics, they can easily cause failures in the physics simulation process and are obvious in the human senses.
To address this issue, our MCM first detects flawed motion, then regenerates the problematic motion segment guided by the motion context and human mask signals, ultimately replacing the flawed motion.
% we replace the broken frames with smooth motions, leveraging the contextual information from the reference motion and mask data derived from segmentation.

\textbf{Mismatch Detection.} 
Given the reference motion and its corresponding video, we project the 3D positions of the reference motion into 2D camera coordinates. Also, an object detection algorithm is used to extract the corresponding 2D keypoints from the video. Using the Object Keypoint Similarity (OKS) algorithm, we compute the matching degree between the two sets of keypoints and obtain a similarity score sequence. Frames with a similarity score below a certain threshold will be flagged as flaw motion. 
% \zyc{what the symbols are? is d the threshold?}
\begin{equation}OKS=\frac{\sum_iexp(-d_i^2/2s^2)\delta(v_i>0)}{\sum_i\delta(v_i>0)}\end{equation}
where $v_i$ represents the visibility flag, $s_i$ denotes the scale factor, and $d_i$ is the distance difference between the projection and the detection results.
Additionally, segmentation algorithms can also be used to detect flaw motion. We project the SMPL-generated mesh onto the 2D plane and treat it as a set of pixel points. 
The matching similarity can be calculated by determining the proportion of projected mesh points that are contained within the human mask.
% The matching similarity can be determined by calculating the Intersection over Union (IoU) similarity between the segmented mask set and the projected mesh set.

% \textbf{Motion Representation.} \zyc{See the latex comments here!}%这部分和下一部分没有写清楚，Motion Representation 是创新吗？不是的话简洁些，是的话这个表示创新在哪里？有啥好处没有写清楚； Mask-conditioned Motion Diffusion In-betweening这里写的不是很好，重点放在训练任务的设计上，为扩散模型设计了什么训练任务，为了达到这一目标对输入的条件进行了哪些操作，目前写的只是怎么做，没有很好突出任务的设计。
% Given a human motion sequence $x \in \mathbb{R}^{N \times D}$, the segmented human mask $m \in \mathbb{R}^{N \times w \times h}$, and a keyframe signal (which identifies frames requiring inbetweening), this module restore the mismatched motion frames. The human motion $x$ is derived from the reference motion, where we compute a 135-dimensional motion representation based on SMPL parameters, which includes 3-dim translation, 6-dim root rotation, and 21 body joint rotations.
% The observation signal is generated from the mismatch detection algorithm.

\textbf{Motion Correction Goal Design.}
Unlike traditional inbetween methods, the goal of the MCM is to replace flawed motions in the reference sequence based on contextual information, ensuring that the corrected reference motion is smooth and continuous. Thus, we focus solely on the model’s ability to fill temporal gaps. Given that the input to the MCM is motion captured from video, it is crucial to ensure that the generated motion remains as consistent as possible with the original video content. To achieve this, we use the human mask obtained from segmentation as a conditional signal to guide the inbetween process.

\textbf{Mask-conditioned Diffusion In-betweening.} 
Given a reference motion sequence $x \in \mathbb{R}^{N \times D}$, the segmented human mask $m \in \mathbb{R}^{N \times w \times h}$, and a keyframe signal (generated from the mismatch detection, identifies frames requiring correction), this module correct the reference motion by replacing mismatched motion frames.
% Before executing the diffusion model \cite{karunratanakul2023gmd,cohan2024flexible}, we use a Vision Transformer (ViT) \cite{alexey2020image} to extract human pose and shape features from the human mask. 
We employ a pre-trained Vision Transformer (ViT) as the mask feature extractor to capture rich human pose information from the segmentation mask.
The extracted features are used as the mask condition for the diffusion process. 
% Only the motion frames that need to be replaced should be subjected to noise, while the remaining parts are retained as the motion context.
% To inform the model which frame can be observed, we also concatenate the resulting sample $x_t$ with the keyframe signal as input to the diffusion model. The image mask features are combined similarly, ensuring that both the temporal keyframes and spatial mask features guide the diffusion process effectively. 
Following \cite{karunratanakul2023gmd,cohan2024flexible}, we concatenate the resulting sample $x_t$, keyframe signal and mask features as model input to inform the generation model with condition signal.

\textbf{Training process.}
We use motion captured from videos as the training data. A random segment of motion, selected at a random position within the entire motion sequence, is chosen as the generation target. Our model is trained to reconstruct this segment. Both keyframe conditioning signals $c$ and mask conditioning signal $m$ are set to $\emptyset$ for 10\% of training samples to make our model suited for unconditioned motion generation.

%\zyc{See LaTeX comments}} %这部分的写法看不出那部分是咱们新提出来的。可以考虑增加：为解决其中什么子问题，提出了什么。

\subsection{Physics-based Motion Transfer Module}
The problem of controlling a humanoid to follow a reference motion sequence $q_{b_{1:T}}$ can be formulated as a Markov Decision Process, defined by the tuple $M = \langle S, A, P_{\text{physics}}, R, \gamma \rangle$, which consists of states, actions, transition dynamics, reward, and a discount factor. 
% The physics simulator provides the state $S$, reward $R$, and transition dynamics $P$, while the policy $\pi_{\text{PTM}}$ determines the action $A$. 
At step $t$, agent selects an action $a_t$ from the policy $\pi_{\text{PTM}}(a_t|s_t)$ based on the current state $s_t$, and the environment responds with the next state $s_{t+1}$ and a reward $r_t$. Proximal Policy Optimization \cite{schulman2017proximal} is used to optimize the policy $\pi^*_{\text{PTM}}$ by maximize the expected discounted return $\mathbb{E}\left[\sum_{t=1}^{T}\gamma^{t-1}r_{t}\right]$.

\textbf{Motion Imitation Formulation.}
The \textbf{state} $s_{t}$ consists of positions, rotations, and linear and angular velocities of humanoid, as well as the next frame information ${g}_t$ from the reference motion.  We define ${g}_t$ as the difference between the next frame reference motion and the current frame humanoid state.
% (use rotation difference for $\mathcal{\theta}_t$). 
Unlike directly using the next frame of the reference motion, leveraging the difference has been shown to effectively inform the policy on compensating for the pose residual \cite{yuan2023physdiff}.
The \textbf{action} $a_t$ specifies the target joint angles for the Proportional-Derivative controller at each degree of freedom (DoF) of the humanoid joints.
Given an action, the torque to be applied is computed as:
\begin{equation}
\tau^i=k_p^i(a_t^i-x_t^i)-k_d^iq_t^i ,
\end{equation}
where $i$ means joint DoF index, $k_p$ and $k_d$ are manually-specified gains. This design helps our method perform better when the reference motion is unreal and noisy \cite{luo2023perpetual}. 
% since our controller is designed to handle repair task.
% \textbf{Policy.} 
% The policy $\pi_{\text{PTM}}$ is represented by a Gaussian distribution with a fixed diagonal covariance matrix. 
% Our policy $\pi_{\text{PTM}}$ utilizes a neural network to map state $s_t$ to the mean $\nu_t$ of the distribution. 
Our \textbf{policy} $\pi_{\text{PTM}}$ is constructed with 6-layer multilayer perceptions and ReLU activation functions. A discriminator from AMP \cite{peng2021amp}, is used to predict whether a given state $s_t$ and action $a_t$ is sampled from the demonstrations $M$ or generated by policy $\pi_{\text{PTM}}$. 
% Our discriminator is an MLP with two hidden layers with ReLU activation function.
% \textbf{Reward.}
The \textbf{reward} has three main components, a reconstruction reward $r_t^\mathrm{g}$ to follow the reference motion, a style reward $r_t^\mathrm{amp}$ produced by the amp discriminator, and energy penalty $r_t^\mathrm{energy}$ \cite{peng2018deepmimic} to prevents motion jitter. 
% as the sum of tracking reward , style reward $r_t^\mathrm{amp}$, and energy penalty $r_t^\mathrm{energy}$ \cite{peng2018deepmimic} :
\begin{equation}r_t=r_t^\mathrm{g}+r_t^\mathrm{amp}+r_t^\mathrm{energy}.\end{equation}

% $rela()$ means to ignore the gravity axis part of root joints. 
% This reward is effective in tracking daily motion but brings problems in facing in-the-wild complex motions.
% The captured reference motion contains error-accumulating roots and jitter poses that need to be repaired, making it detrimental to construct a full reconstruction reward. Therefore, we designed a relative reward that , maintaining global orientation and translation information through explicit guidance from rotation and implicit guidance from velocity. % neglects the absolute root position of the rigid body

\textbf{Training.} Through the definition of state, action, policy, and reward, we have a controller for physical motion refinement. This controller is pre-trained on both the mocap dataset AMASS and the video motion capture results of AIST++ and Kungfu (train set). The reference motion often exhibits cumulative errors such as ground penetration and floating during prolonged displacements. The present of gravity and ground in the physical environment exacerbates their impact, significantly hindering the training process. To address this, we designed a motion pre-processing method and implemented segmented training for long sequences, reinitializing the starting position for each segment.
% , with strict reconstruction rewards and distance-based experiments termination

\textbf{RL-based Test Time Adaptation}
% Current video motion capture methods can generate surprisingly complex motions, particularly in in-the-wild videos. 
% However, it remains highly challenging to project these motions into the physical space through post-processing motion restoration.
% Due to the inherent generalization limitations of reinforcement learning, a purely PTM still struggles to handle in-the-wild motions. 
% This approach enables the repair of physical realism in high-difficulty in the wild motions.
With a pre-trained imitation controller, rich motion priors open up the possibility for rapid adaptation during test time. Utilizing the trial-and-error nature of reinforcement learning, we propose RL-based test time adaptation, which involves performing a limited number of experiment steps on the current test data under specific adaptation settings (updating network parameters). Each motion sequence is treated as an individual instance, and the adaptation is performed for each instance independently. This method is particularly useful when dealing with high-difficulty and low-quality motions. The following designs are used in the adaptation process.
% In addition to the challenges of generalization, high-difficulty motions differ from daily motions in several key ways:
% 1) Complex airborne poses.
% 2) Rapidly shifting root positions.
% 3) Extreme body postures.
% Our method addresses these issues through the following design.

\textbf{Relative Reward.}
% To ensure accurate reproduction of the reference motion, the motion simulation strategy
% Motion tracking methods typically construct a multi-dimensional reward to encourage the model to align closely with the reference, which usually includes position, rotation, velocity, and angular velocity. 
% guide the humanoid’s reconstruction from various perspectives, 
% These components imposing strong constraints on the motion simulation, which trap the model in the minutiae of reconstruction, slowing or even stalling the overall tracking process.
% . However, such strict constraints can
% In physical motion restoration tasks, 
 %, making it hard to follow.
% meaning we don't need to fully follow the reference motion. 
The captured reference motion contains error-accumulating roots and jitter poses that need to be repaired, making it detrimental to construct a full reconstruction reward.
Therefore, in adaptation process, we designed a relative reward that neglects the absolute root position, maintaining global orientation and translation through explicit guidance from rotation and implicit guidance from velocity. The relative reward is formulated as: 
\begin{equation}
\begin{aligned}&r_{t}^{\mathrm{g}}=w_{\mathrm{p}}e^{-100\|rela(\boldsymbol{\hat{p}}_{t})-rela(\boldsymbol{p}_{t})\|}+w_{\mathrm{r}}e^{-10\|\boldsymbol{\hat{\theta}}_{t}\ominus\boldsymbol{\theta}_{t}\|}\\&+w_{\mathrm{v}}e^{-0.1\|\boldsymbol{\hat{v}}_{t}-\boldsymbol{v}_{t}\|}+w_{\mathrm{\omega}}e^{-0.1\|\boldsymbol{\hat{\omega}}_{t}-\boldsymbol{\omega}_{t}\|},\end{aligned}
\end{equation}
where $\boldsymbol{\hat{p}}_{t}$ means the joint position of reference motion, $rela()$ means to ignore the gravity axis part of root joints. $\ominus$ means rotation difference.
% The overall reward is defined as the sum of tracking reward $r_t^\mathrm{g}$, style reward $r_t^\mathrm{amp}$, and energy penalty $r_t^\mathrm{energy}$ \cite{peng2018deepmimic}:
% \begin{equation}r_t=0.5r_t^\mathrm{g}+0.5r_t^\mathrm{amp}+r_t^\mathrm{energy}.\end{equation}
% allowing the model to restore the motion while disregarding unreasonable root movement and jitter. The humanoid's global orientation and displacement are maintained through explicit guidance from rotation and implicit guidance from velocity.


% To improve training efficiency and prevent undesirable behaviors or unstable states, early termination is often employed during policy training. The distance termination condition proposed in UHC performs well in many tasks. However, in high-difficulty motion simulations, frequent floating and aerial movements often prematurely trigger distance termination.
% Therefore, we modified the distance termination based on relative position and introduced early termination conditions based on joint height and ground contact, ensuring its applicability to complex motions while preserving its advantages. The relative position adjustment reduces sensitivity to floating and jitter, allowing the model to focus more on the motion itself. The ground contact condition further refines failure boundaries in ground interactions, which are critical for high-difficulty motions involving complex ground interactions, such as yoga and breakdancing.

% Since high-difficulty reference motion often involves frequent floating and aerial movements, making the displacement between humanoid
\textbf{Early Termination.} In high-difficulty motion tracking, there is a large displacement between humanoid and reference motion, as reference motion often involves frequent floating and penetration. This phenomenon makes defining when an experiment should be terminated challenging, which is crucial for training efficiency and preventing undesirable behaviors. Therefore, we design a relative termination condition by calculating each joint's mean relative distance between humanoid and reference motion.
% , assuming their roots coincide at a single point. 
Experiments will be terminated when the distance is larger than threshold $d_{term}$. We also introduce termination condition $\mathcal{F}^h_t$ and $\mathcal{F}^c_t$ based on joint height and ground contact to end the experiments when falls and erroneous contacts occur. The full termination $\mathcal{F}_t$ is defined below, a smaller threshold $d_{term}$ indicating a stricter adherence to reference motion.
\begin{equation}
    \mathcal{F}_t = \left( \frac{1}{J} \sum_{i=1}^{J} \|rela(\boldsymbol{\hat{p}}^{i}_{t})-rela(\boldsymbol{p}^{i}_{t})\| > d \right) \vee \mathcal{F}^h_t \vee \mathcal{F}^c_t
\end{equation} 
 

% \zyc{How to get the threshold $d$? } %这个阈值的设定是根据什么设计的，不同数据之间是否有差异？

\textbf{Residual Force.} During the test-time adaptation phase, we introduce residual forces \cite{yuan2020residual} to compensate for the dynamics mismatch.
% and more effectively imitate the reference motion. 
This is important because complex motions often involve airborne flips and jumps (commonly seen in gymnastics and martial arts), which frequently rely on elastic trampolines and mats for execution. The use of external forces is necessary to account for the absence of these environmental conditions in our simulations.
% Since the motion restoration scenarios involve a wider variety of force application points (e.g., hand support in handstands, waist control in backflips, and footwork in ballet), we define residual forces on all joints of the humanoid. 
% Additionally, we relax the regularization constraints on these external forces to allow for greater flexibility in addressing the specific force requirements of different motions.

% \textbf{Test-Time Adaptation.} In practical applications, our test-time adaptation approach can be implemented in two distinct forms. The first is Source-Free Domain Adaptation, which involves adapting our model within a certain amount of data,
% % randomly sampling data prior to testing for domain fitting, 
% allowing the model's capabilities to be transferred across the entire dataset. This approach is suitable for optimizing low-difficulty motions within specific subdomains.
% The second form is Test-Time Instance Adaptation, where each motion sequence is treated as an individual instance, and the adaptation is performed for each instance independently. This method is particularly useful when dealing with high-difficulty and low quality motions.
% when the reference motion data is of low quality.

\subsection{Implementation details}
% Our model can be trained on a single NVIDIA A100 GPU and I
It takes around 2-3 days to get our pre-trained PTM with a single NVIDIA A100 GPU. During inference, restoring normal motions (such as running, and jumping) requires fewer adaptation steps (less than 500) or may not require any adaptation at all. In contrast, restoring high-difficulty motions (such as continuous rolls and aerial maneuvers) necessitates between 2,000 and 4,000 steps, depending on the complexity of the motion and the quality of the reference action. We adopt the motion diffusion model GMD with UNet architecture as our in-between baseline \cite{dhariwal2021diffusion,ho2020denoising}. For more implementation details, please refer to the Appendix.





==> backup/related1114.tex <==
\section{Related Work} 
\label{sec:related}

\begin{figure*}[t]
\vspace{-25pt}
    \centering
\includegraphics[width=0.8\textwidth, height=0.28\textwidth]{picture/pipeline6.png}
    \caption{\label{fig:pipeline}\textbf{Illustration of our proposed method.} If no mismatch is detected between the human mask and noise motion, the correction process will be skipped, and our PTM directly takes the noise motion as input.
    When failed with challenge motions, our PTM will adapt the policy to the current motion and update the network parameters until success or reach a certain step threshold. 
    }
     \vspace{-5mm}
\end{figure*}
 

\subsection{Video Motion Capture}
% The most common approach
Most works for video motion capture are to recover the parameters of a parametric human model \cite{loper2023smpl,kanazawa2019learning,choi2021beyond, kocabas2020vibe,luo20203d,sun2019human,shen2023global}. 
% Given a single image or video, the goal is to align the human mesh with 2D images.
% Many works based on the HMR pipeline and improve it by incorporating convolutional encoders \cite{kanazawa2019learning}, RNNs \cite{choi2021beyond, kocabas2020vibe,luo20203d}, self-attention mechanisms in CNNs \cite{sun2019human}, and transformer encoders \cite{shen2023global}.
% In optimization-based approaches, the SMPL model can be fitted to images [1, 7, 15, 71], videos [3, 23, 89], and other sensing modalities [81, 88] through energy minimization.
% The continuous improvement in accuracy is partly due to advancements in datasets \cite{black2023bedlam,joo2021exemplar,von2018recovering}, and partly from the clever design of architectures that incorporate domain knowledge \cite{von2018recovering}.
% Recently, many methods have incorporated moving cameras into consideration.
Recently, many methods have started to consider moving cameras.
% , but recovering global positions from in-the-wild videos remains challenging. 
TRACE \cite{sun2023trace} and WHAM \cite{shin2024wham} propose regressing per-frame poses and translations.
% , achieving significant results by learning trajectory regression from motion capture data.
SLAHMR \cite{ye2023decoupling} and PACE \cite{kocabas2024pace} integrate SLAM \cite{teed2021droid,teed2024deep} with pre-learned motion priors \cite{rempe2021humor} into the optimization framework.
TRAM \cite{wang2024tram} leverages the scene background to derive motion scale.
% and converting the camera coordinates into a world coordinate.
GVHMR \cite{shen2024world} estimates human poses in a novel Gravity-View coordinate system.
While these methods achieve significant success in reconstructing high-difficulty motions from videos, they suffer from serious physical issues and occasionally experience flawed motions when facing complex movements.
% do not account for physical constraints, leading to serious physical issues.
% , such as foot sliding, floating, and penetration. 
% Additionally, video motion capture methods occasionally experience flawed motions when facing complex movements. 
Our proposed physical motion restoration method effectively addresses these problems.

\subsection{Physics informed Video Motion Capture}
% Researchers have introduced physics-based optimization methods to address the challenge of ensuring physical plausibility in estimated human motion. 
Many researchers attempt to introduce physics into video motion capture.
Learning-based methods \cite{shimada2021neural,huang2022neural,gartner2022trajectory,tripathi20233d} leverage neural networks to estimate physical parameters for motion capture and introduce the kinematic constrains to enhance the physical plausibility. LEMO \cite{zhang2021learning} uses motion smoothness prior and physics contact friction term. Xie ~\etal \cite{xie2021physics} propose differentiable physics-inspired objectives with contact penalty. IPMAN \cite{tripathi20233d} exploits intuitive-physics terms to incorporate physics. Li ~\etal \cite{li2022d} enhanced the learning process by incorporating 3D supervision. 
% However, existing learning-based methods often use oversimplified physics equations with rely on 3D annotated videos, and often struggle with generalization to out-of-distribution motions.
Learning-based methods typically require hard-to-obtain 3D annotations and overly simplify dynamic equations, struggling with generalization to out-of-distribution motions.
% A method more similar to our task is PhysPT, which employs self-supervised learning and uses a Physics-aware Pretrained Transformer to improve kinematics-based motion estimates. However, PhysPT primarily focuses on optimizing relatively simple motions and struggles to correct high-difficulty actions, often resulting in physically unrealistic outcomes for more complex movements. In contrast, our approach offers a plug-and-play solution for enhancing the physical realism of diverse and challenging motions. It is not limited to specific action tasks and does not rely on 3D annotated videos for training, making it more versatile and robust for a wider range of applications.
Optimization-based  methods treat the captured motion as a reference and predict the physical simulation forces with a controller \cite{yuan2021simpoe,gong2022posetriplet,zhang2024proxycap}. 
DiffPhy \cite{gartner2022differentiable} uses a differentiable physics simulator during inference. 
PhysCap \cite{shimada2020physcap} uses a numerical optimization framework with soft physical constraints.
SimPoE \cite{yuan2021simpoe} integrates image-based kinematic inference and physics-based dynamics modeling.
However, these methods typically require careful tuning of control parameters and are sensitive to different motion types \cite{huang2022neural}. 
This sensitivity makes it challenging to generalize to in-the-wild high-difficulty motions, limiting real-world applications.
% Another class of learning-based methods leverages neural networks to estimate physical parameters for motion generation [3D Human Pose Estimation via Intuitive Physics]. Xie et al. [Physics-based human motion estimation and synthesis from videos] propose differentiable physics-inspired objectives based on a soft contact penalty. IPMAN exploits novel intuitive-physics (IP) terms to take physics into account [3D Human Pose Estimation via Intuitive Physics]. Li et al. [DD: Learning Human Dynamics from Dynamic Camera] enhanced the learning process by analytically computing certain physical parameters and incorporating 3D supervision. However, existing learning-based methods typically rely on 3D annotated videos and often struggle with generalization to out-of-distribution motions.
Recently, PhysPT \cite{zhang2024physpt} proposed a pre-trained physics-aware transformer to learn human dynamics in a self-supervised manner. % into motion estimates. 
However, it lacks an understanding of the distribution and physical rules of high-difficulty motions, necessitating additional physical priors of complex motions, which is challenging due to data scarcity. 
% PhysPT cannot process flaw motions and, due to its root translation re-prediction, it struggles to get a faithful reconstruction of the original motion. 
In contrast, our approach is designed to restore high-difficulty and in-the-wild motions while maintaining their original motion pattern.
% tackle high-difficulty motions, capable of
% A method more similar to our task is PhysPT, which employs self-supervised learning and uses a Physics-aware Pretrained Transformer to improve kinematics-based motion estimates. However, PhysPT primarily focuses on optimizing relatively simple motions and struggles to correct high-difficulty actions, often resulting in physically unrealistic outcomes for more complex movements. In contrast, our approach offers a plug-and-play solution for enhancing the physical realism of diverse and challenging motions. It is not limited to specific action tasks and does not rely on 3D annotated videos for training, making it more versatile and robust for a wider range of applications.



\subsection{Motion Imitation}
The physical constraints provided by simulation environments give simulated characters a clear advantage in generating lifelike human movements \cite{peng2018deepmimic,peng2017deeploco,peng2019mcp,peng2022ase,peng2021amp,chentanez2018physics,merel2020catch,winkler2022questsim,gong2022posetriplet,fussell2021supertrack}.
% Due to the non-differentiable nature of modern physics simulators, we rely on reinforcement learning to train these simulated agents.
Early works focused on small-scale task-specific scenarios and are difficult to generalize to other domains.
With the advancements in motion generation technology, training policies to imitate large-scale motion datasets show broader application potential. 
% These simulation policies can be easily paired with motion generators to achieve various tasks. 
Researchers improve motion simulation quality by leveraging techniques such as hybrid expert policies \cite{won2020scalable}, differentiable simulation \cite{ren2023diffmimic}, and external forces \cite{yuan2020residual}.
ScaDiver \cite{won2020scalable} extended the hybrid expert strategy to the CMU motion capture dataset. Unicon \cite{wang2020unicon} demonstrated qualitative results in imitation and transfer tasks.
% but did not quantify the policy’s ability to imitate specific dataset segments. 
MoCapAct \cite{wagener2022mocapact} learn a single-segment expert policy on the CMU dataset. 
UHC \cite{luo2021dynamics} successfully imitated 97\% of the AMASS dataset, and more recently, PHC \cite{luo2023perpetual} enabled a single policy to simulate almost the entire AMASS dataset while allowing recovery from falls.
However, these methods rely heavily on the quality of reference motions and are largely confined to locomotion tasks. 
% making it challenging to simulate more diverse and high-difficulty data.
% Due to the limitations in the generalization capability, 
Simulating in-the-wild and high-difficulty motions is still challenging, where our proposed PTM provides a possible solution.

 




==> sec/finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/intro_cvpr.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/sup.tex <==
\begin{figure*}[t]
    \centering
\includegraphics[width=\textwidth]{picture/before_after1.png}
    \caption{\label{fig:before_after}\textbf{Visualization of the high-difficulty motions before and after our physical restoration .} }
\end{figure*}

\begin{figure*}[t]
    \centering
\includegraphics[width=\textwidth]{picture/sup_class2.png}
    \caption{\label{fig:class1}\textbf{Visualization of the in-the-wild and high-difficulty motions restored from our method (1/2).} }
    \vspace{10mm}
\end{figure*}

\begin{figure*}[t]
    \centering
\includegraphics[width=\textwidth]{picture/sup_class1.png}
    \caption{\label{fig:class2}\textbf{Visualization of the in-the-wild and high-difficulty motions restored from our method (2/2).} }
\end{figure*}

\begin{figure*}
    \centering
\includegraphics[width=\textwidth]{picture/flaw_motion.png}
    \caption{\label{fig:flaw}\textbf{Additional cases of flawed motion.} }
\end{figure*}

\begin{figure*}
    \centering
\includegraphics[width=\textwidth]{picture/sup_compare1.png}
    \caption{\label{fig:compare}\textbf{Additional comparison with SOTA techniques.} }
\end{figure*}

\section{Additional Visualization}
\textbf{Physical Restoration Visualization.} In Figure \ref{fig:before_after}, we select high-difficulty in-the-wild motions (taekwondo and rhythmic gymnastics) and illustrate a comparison before and after our restoration.
% across different reference motions. We selected high-difficulty in-the-wild motions, such as taekwondo and rhythmic gymnastics. 
As shown in the figure, our method effectively eliminates issues of ground penetration and floating in the original motions, successfully transferring the raw movements into physical space. 
% Despite the original motions containing complex sequences of inversions, rolls, and mid-air rotations that are challenging to reproduce in physical space, our motion correction method maintains these motion characteristics. 
Despite the original motions containing multiple continuous complex actions that are challenging to reproduce in physical space, our method effectively eliminates issues of ground penetration and floating in the original motions while successfully maintaining the original motion patterns. 
Notably, our method has never seen taekwondo or rhythmic gymnastics motions before, which underscores the strong generalization ability of our method.

\textbf{Visualization of different motion types.} In Figures \ref{fig:class1} and \ref{fig:class2}, we demonstrate the performance of our method on various types of challenging motions, including Taekwondo, Chinese kungfu, breakdancing, rhythmic gymnastics, and ballet. The visualized results show that our method can effectively perform physics-based motion restoration for a diverse range of high-difficulty movements, producing high-fidelity motions to the original video. Notably, our training dataset does not include such a wide variety of complex motions, nor does it rely on any expensive 3D annotations, which further proves the effectiveness and broad applicability of our approach.

\textbf{Flaw Motion Cases.} In Figure \ref{fig:flaw}, we provide additional cases of flawed motion shown in the advanced video motion capture method GVHMR \cite{shen2024world}, flawed motion usually happens from the rapid and extreme movement of high-difficulty motions and the blurred frames. Our method successfully corrected these flawed motions and converted them to physical realism motions.

\textbf{Additional SOTA Comparison.} In Figure \ref{fig:compare}, we provide additional visual comparisons with state-of-the-art methods (gymnastics and yoga). The performance of each method on different types of motions is consistent with the visual comparisons presented in the main text. Due to limitations in generalization, PHC+ \cite{luo2023universal, luo2023perpetual} struggles to simulate high-difficulty movements, resulting in falls during the simulation. PhysPT \cite{zhang2024physpt}, due to its simplified physical constraints, avoids falling during the restoration process, but its physical repair ability is limited when facing high-difficulty motions. It still suffers from issues related to physical realism and struggles to maintain the original motion patterns of the reference motions. In the first row of Figure \ref{fig:compare}, the ground in the motion generated by GVHMR appears somewhat unusual as we calculate it with the mean operation. This is because we need to display the entire motion in the visualization. We do not use this approach in other visualizations and metric calculations. Instead, we calibrate the ground based on the foot position in the first frame.




\section{Motion Inbetweening}
 \textbf{Motion Representation.}
%在虚拟环境中，我们使用更加完备的表征来定义仿真环境中的humanoid以进行更加细粒度的控制，但这种motion表征对动作生成而言是冗余的。因此，在MCM中我们采用了更简单的表征定义，依然保证其与SMPL格式的方便转换。
% In the virtual environment, we use a more comprehensive representation to define the humanoid for finer-grained control in simulation. However, this motion representation is redundant for motion generation purposes. Therefore, 
In the Mask-conditioned Motion Correction Module (MCM), we adopt a simpler representation that ensures convenient conversion to the SMPL \cite{loper2023smpl} format.
Given a human motion sequence $\boldsymbol{x} \in \mathbb{R}^{N \times D}$, the segmented human mask $\boldsymbol{m} \in \mathbb{R}^{N \times w \times h}$, and a keyframe signal (which identifies frames requiring inbetweening), this module restore the mismatched motion frames. The human motion $\boldsymbol{x}$ is derived from the reference motion, where we compute a 135-dimensional motion representation based on SMPL parameters, which includes 3-dim translation, 6-dim root rotation, and 21 body joint rotations.
The observation signal is generated from the mismatch detection algorithm.

\textbf{Motion Inbetween with Diffusion Models.}
%扩散模型在生成模型中表现出了令人印象深刻的性能，最近，diffusion probabilistic models被引入到3D人体动作生成之中，将动作生成视为一种序列生成问题。motion inbetween是3D人体动作生成的子任务，相比于普通的动作生成，inbetween不从直接从噪声中还原整段motion，而是为扩散模型提供motion的一部分作为条件，inbetween的目标是生成motion中缺失的部分。通常，motion会在某种条件的指导下生成（如文字，音乐或者图片），这些条件也可以用于inbetween任务。在此文中。我们采用分割得到的人体mask作为条件（本质上是图像的简化版本，利用当前分割模型的强大先验减轻inbetween模型的负担）。在人体mask的指导下，扩散模型利用去噪网络来学习Gaussian noise的去噪过程。
Diffusion models have demonstrated impressive performance in generative modeling, and recently, diffusion probabilistic models have been introduced into 3D human motion generation, framing motion generation as a sequence generation problem. Motion inbetween is a subtask of 3D human motion generation. Unlike regular motion generation, inbetween does not directly reconstruct the entire motion from noise but provides a partial motion as a condition for the diffusion model. The goal of inbetween is to generate the missing part of the motion. Typically, motion is generated under certain conditions (such as text, music, or images), and these conditions can also be used for the inbetween task. In this work, we use the human body mask obtained from segmentation as a condition (essentially a simplified version of the image, leveraging the powerful priors of current segmentation models to alleviate the burden on the inbetween model). Guided by the human mask $\boldsymbol{m}$, the diffusion model uses a denoising network to learn the process of denoising Gaussian noise.
\begin{equation}p_\theta(\boldsymbol{x}_{t-1}|\boldsymbol{x}_t,\boldsymbol{m}):=\mathcal{N}(\boldsymbol{x}_{t-1};\boldsymbol{\mu}_\theta(\boldsymbol{x}_t,t,\boldsymbol{m}),\Sigma_t)\end{equation}
where $\theta$ demonstrates the parameters of the denoising network and the untrained time-dependent covariance is set according to the variance schedule. Following current motion generation methods, we use sample-estimation reparameterization and directly predict the clean sample estimate from noise, rather than the mean estimate. The training goal of the diffusion model can be defined as:
\begin{equation}\mathcal{L}:=\mathbb{E}_{(\boldsymbol{x}_0,\boldsymbol{m})\sim q(\boldsymbol{x}_0,\boldsymbol{m}),t\sim[1,T]}\left[\|\boldsymbol{x}_0-G_\theta(\boldsymbol{x}_t,t,\boldsymbol{m})\|^2\right].\end{equation}
%表示去噪网络的参数，untrained time-dependable covariance set according to the variance schedule. Following当前的动作生成方法，我们use the sample-estimation reparameterization and directly predict the clean sample estimate from noise，而不是mean estimate。在我们的目标下，扩散模型的训练目标可以定义为：


\textbf{Auxiliary Losses}
%除了基本的重建损失，We introduce several auxiliary losses to enhance training stability。由于我们采用了基于旋转的动作表征，我们在计算其他loss之前需要recover得到人体的global position。In addition to the reconstruction loss Lsimple, we adopt Loss of joint positions.
In addition to the basic reconstruction loss, we introduce several auxiliary losses to enhance training stability. Since we adopt a rotation-based motion representation, we need to recover the global position of the human body before computing the other losses. We incorporate a loss on joint positions.
\begin{equation}\mathcal{L}_{\mathrm{joint}}=\frac1J\sum_{i=1}^J\|FK(\boldsymbol{x}^{(i)})-FK(\boldsymbol{\hat{x}}^{(i)})\|_2^2\end{equation}
where $FK$ means the forward process for motion representation to get the absolute 3D position $\boldsymbol{p}$. $\boldsymbol{\hat{x}}$ and $\boldsymbol{\hat{p}}$ is obtained from the model prediction.
To enhance the smoothness of the generated motion, we introduce a velocity loss and an acceleration loss.
\begin{equation}\mathcal{L}_{\mathrm{vel}}=\left\|\boldsymbol{p}_{\mathrm{vel}}-\hat{\boldsymbol{p}}_{\mathrm{vel}}\right\|_{2}^{2},\mathcal{L}_{\mathrm{acc}}=\left\|\boldsymbol{p}_{\mathrm{acc}}-\hat{\boldsymbol{p}}_{\mathrm{acc}}\right\|_{2}^{2},\end{equation}
Additionally, to improve the accuracy of root position generation, we introduce extra constraints on both the root translation and orientation.
% \begin{equation}\mathcal{L}_{RO}=||O(\boldsymbol{x},\hat{\boldsymbol{x}})-O(\boldsymbol{x},\boldsymbol{x})||_2^2,\end{equation}
\begin{equation}\mathcal{L}_{\mathrm{ro}}= \left\|\boldsymbol{x}^{ro}-\hat{\boldsymbol{x}}^{ro}\right\|_{2}^{2} + \left\|\boldsymbol{x}_{\mathrm{vel}}^{ro}-\hat{\boldsymbol{x}}_{\mathrm{ro}}^{ro}\right\|_{2}^{2}+\left\|\boldsymbol{x}_{\mathrm{acc}}^{ro}-\hat{\boldsymbol{x}}_{\mathrm{acc}}^{ro}\right\|_{2}^{2},\end{equation}
where $\boldsymbol{x}^{ro}$ is 7-dim orientation and translation of motion $\boldsymbol{x}$.


\section{Implementation Details}
\textbf{Training} 
Our method consists of two modules, MCM and PTM, which are trained separately.
For the Mask-conditioned Motion Correction Module, we select the ground truth data from the Human3.6M \cite{ionescu2013human3}, AIST++ \cite{li2021learn,aist-dance-db}, and Motion-X \cite{lin2023motionx} Kungfu datasets as the training set. Additionally, we use SAM \cite{kirillov2023segany} to process these datasets and generate the corresponding mask data. The mask data serves as a condition to guide the motion correction process.
For the Physics-based Motion Transfer Module, we use the AMASS \cite{mahmood2019amass}, Human3.6M, AIST++, and Kungfu datasets for training. 
% It is worth noting that the AIST++ and Kungfu datasets, which are also estimated from videos, suffer from various issues such as penetration and floating problems in their ground truth data. Therefore, we apply a preprocessing method \cite{tseng2023edge}, to optimize the foot-ground contact before using these datasets. The key idea is to identify frames where the horizontal velocity of the foot joint is small, marking them as contact frames, and then reset the foot positions to the ground. Moreover, to prevent the accumulation of errors in long-duration data, we split the long training sequences into segments and reset the body position at the start of each segment to a standard reference position. %This ensures that the motion transfer process is stable and consistent over extended periods of time.
% However, this does not imply that 
Our method is not limited to a fixing short-motion clip, on the contrary, our approach supports long-duration motion repair. The repair capability depends on the quality of the reference motion and the complexity of the action, rather than the length of the motion sequence.

\textbf{Imitation} 
Our simulation environment is NVIDIA’s Isaac Gym \cite{makoviychuk2021isaac}, where the humanoid model is adapted to a format compatible with SMPL, as it natively supports various body shapes and is widely used in pose estimation research. As a result, our restoration outputs can be easily converted to the SMPL format and rendered into realistic meshes. Currently, we do not consider complex SMPL body shapes in our approach. Our discriminator is an MLP with two hidden layers with ReLU activation function. The policy of our PTM is constructed with 6-layer multilayer perceptions and ReLU functions.




\textbf{Metrics Details}
%此小节中，我们将从物理真实性和2D相似性两个方面讨论我们提出的测试基准。在物理真实性方面，我们使用了1) Self-Penetration (SP), SP是指人体动作表征渲染得到的SMPL mesh中部分表面顶点出现在了mesh内部，比较常见的是手指穿过腰部。我们计算每一帧中出现在人体mesh内部的顶点占全部顶点的比例，并将比例在时间维度上的平均值作为子穿模指标。2) Ground-Penetration (GP), GP是指人体动作表征渲染得到的SMPL mesh中部分顶点出现在地面下方，we compute the distance between the ground and the lowest body mesh vertex below the ground. 3) Float指人体SMPL mesh中所有顶点都在地面上方，following xx, we compute the distance between the ground and the lowest body mesh vertex above the ground. 在计算过程中GP和Float都采用了5mm的阈值，低于此阈值的GP和Float将被忽略。4) Foot-Skate (FS), 我们找出两个相邻帧中与地面接触的脚关节，并计算它们在帧间的平均水平位移。在2D相似性方面，我们使用了1) 2D关键点OKS, 我们根据动作表征计算3D绝对位置，随后将3D坐标投影的2D图片上，计算3D投影与2D标注之间的OKS。为了与更多的2D/3D关键点表示适配，OKS的计算采用了12个关键点，分别是left/right hip, knee, ankle, shoulder, elbow, wrist. 2) Mask-Pose Similarity (MPS), 为了更加细粒度的描述动作并将人体shape考虑在内，我们提出了MPS来计算人体mesh的2D投影与人体图片分割的相似度，MPS通过计算落在人体分割mask中的3D mesh顶点的比例得到。A larger ratio signifies higher motion 2D similarity and a more accurate human shape estimation.
In this section, we discuss the evaluation benchmarks we proposed from two aspects: physical realism and 2D similarity. For physical realism, we use the following metrics:
\begin{itemize}
\item Self-Penetration (SP): SP means some surface vertices of the SMPL mesh (rendered from the human motion representation) appear inside the mesh, such as fingers passing through the torso. We calculate the proportion of vertices that penetrate the body mesh in each frame and average this ratio over time as the self-penetration metric.

\item Ground-Penetration (GP): GP refers to vertices of the SMPL mesh that appear below the ground. We compute the distance between the ground and the lowest body mesh vertex that is below the ground.

\item Float: Float happens when all body mesh vertices are above the ground. Following \cite{yuan2023physdiff}, we calculate the distance between the ground and the lowest body mesh vertex above the ground. Both GP and Float use a 5mm threshold, with values below this threshold being ignored.

\item Foot-Skate (FS): We identify the foot joints in two adjacent frames that are in contact with the ground, and then calculate their average horizontal displacement across frames.
\end{itemize}
For 2D similarity, we use the following metrics:
\begin{itemize}
\item 2D Keypoint OKS: We first compute the 3D absolute positions from the motion representation, then project these 3D coordinates onto the 2D image plane. The 2D Keypoint OKS is then calculated as the similarity between the 3D projections and the 2D annotations. To ensure compatibility with various 2D/3D keypoint representations, the OKS calculation uses 12 keypoints: left/right hip, knee, ankle, shoulder, elbow, and wrist. The 2D annotations is obtained from multiple advanced keypoints detection methods and we corrected them manually.

\item Mask-Pose Similarity (MPS): To provide a more granular description of the motion and take into account the human shape, we introduce MPS to calculate the similarity between the 2D projection of the human mesh and the segmentation mask of the human body in the image. MPS is calculated by determining the ratio of 3D mesh vertices within the human segmentation mask. A larger ratio indicates higher 2D similarity and more accurate human shape estimation.
\end{itemize}


\begin{figure}
    \centering
\includegraphics[width=\linewidth]{picture/userstudy.png}
    \caption{\label{fig:userstudy}\textbf{The physical restoration user study of high-difficulty and in-the-wild motions.} }
\end{figure}

\begin{figure}
    \centering
\includegraphics[width=\linewidth]{picture/user_describe2.png}
    \caption{\label{fig:screenshot}\textbf{Screenshot of user study.} }
\end{figure}



%在图1和图2中，我们展示了我们的方法在多种不同类型的高难度动作中的表现，动作类型包含跆拳道，中国武术，霹雳舞，艺术体操，芭蕾舞。可视化结果证明了我们的方法可以对多样化的高难度动作进行物理真实性修复，并得到还原度很高的动作。我们的训练集中并不包含如此多复杂的运动，也无需依赖任何高成本的3D注释，这证明了我们方法的有效性和广泛的应用潜力。
%在图3中，我们提供了额外的与SOTA方法的可视化对比，选取的动作是平面艺术体操和瑜伽。由图可知，各个方法在不同运动类型的表现与正文中的可视化对比一致。由于泛化能力的限制，PHC+难以对高难度动作进行模拟，往往会在模拟中途失败并摔倒。由于简化的物理约束，PhysPT在修复过程中不会出现摔倒，但其修复能力有限，物理真实性问题依然存在，并且难以保持参考动作的原始运动模式。
%图3中第一行GVHMR得到的motion的地面看起来有些奇怪，这是因为我们需要在可视化中完整展示整个动作，在其他可视化和指标计算中我们并不这样做，而是根据第一帧的脚位置来标定地面。

% Figure X demonstrates the role of our designed inbetween module. The upper section shows complex motions directly estimated from video using the advanced GVHMR method, where discrepancies with the human motion in the video occur at frames t3 and t4 (highlighted in red). For clarity, we projected the 3D coordinates onto 2D. Our inbetween module leverages contextual information and the human mask to correct these mismatched frames, producing a smoother, more coherent motion sequence (highlighted in blue).




% \section{Ground Truth Comparison}

%我们的模拟环境是NVIDIA’s Isaac Gym, 模拟环境中的humanid采用了可以与SMPL适配的格式，as it has native support for different body shapes and is widely adopted in the pose estimation literature。因此我们的修复结果可以方便的转换为SMPL格式并渲染成逼真的mesh。目前，我们并没有考虑复杂的SMPL人体shape。
%我们方法的两个模块，MCM和PTM是分开训练的，对于Mask-conditioned Motion Correction Module，我们选取human3.6M, AIST++, kungfu三个数据集的GT数据作为训练集，同时，我们使用SAM处理上述数据集以得到mask数据。对于Physics-based Motion Transfer Module，我们采用AMASS，human3.6M, AIST++, kungfu四个数据集进行训练，值得一提的是，由于AIST++, kungfu数据集也是从视频中估计得到的，他们的GT数据也存在不同程度的穿模和浮空问题。因此，在使用这些数据之前，我们follow edge采用了预处理方法来优化他们的脚和地面接触。主要思想是将脚关节水平速度很小的帧记为接触帧，并将这些帧的脚重置到地面上。此外，为了防止长数据中错误的累积，我们将长时间的训练数据分割为段，并将段首人体的位置转移至标准位置。
%但这不意味着我们的方法只能局限在短时间的motion clip的修复，相反，我们的方法支持长时间的动作修复，修复能力取决与参考动作的质量和动作难度，而不是时间长度。
%除了AMASS数据集，其他数据均采用video motion capture结果作为训练数据，由于video captured motion可能存在flaw motion，我们在使用这些数据之前，先使用MCM进行了flaw motion的去除。

\section{User Study}
To obtain subjective evaluations of different methods, we recruited 44 participants to watch 30 pairs of videos, with one video produced by our method and the other by GVHMR, PhysPT, or PHC+. For each pair of videos, we asked participants to answer three questions: \textit{which video was of better overall quality? Which video has better physical realism? Which video is more restored to the original video?} Thus we ended up with 3960 comparisons.
For each comparison, we asked participants to choose between three options, \textit{the first being better, the second being better, or both being about the same}. The evaluation results are shown in Figure \ref{fig:userstudy}, our method outperforms all other methods in more than 70\%, and only in less than 20\% of the cases are we defeated by other methods.



